ML Based Lineage in Databases

We track the lineage of tuples throughout their database lifetime. That is, we consider a scenario in which tuples (records) that are produced by a query may affect other tuple insertions into the DB, as part of a normal workflow. As time goes on, exact provenance explanations for such tuples become deeply nested, increasingly consuming space, and resulting in decreased clarity and readability. We present a novel approach for approximating lineage tracking, using a Machine Learning (ML) and Natural Language Processing (NLP) technique; namely, word embedding. The basic idea is summarizing (and approximating) the lineage of each tuple via a small set of constant-size vectors (the number of vectors per-tuple is a hyperparameter). Therefore, our solution does not suffer from space complexity blow-up over time, and it "naturally ranks" explanations to the existence of a tuple. We devise an alternative and improved lineage tracking mechanism, that of keeping track of and querying lineage at the column level; thereby, we manage to better distinguish between the provenance features and the textual characteristics of a tuple. We integrate our lineage computations into the PostgreSQL system via an extension (ProvSQL) and extensive experiments exhibit useful results in terms of accuracy against exact, semiring-based, justifications, especially for the column-based (CV) method which exhibits high precision and high per-level recall. In the experiments, we focus on tuples with \textit{multiple generations} of tuples in their lifelong lineage and analyze them in terms of direct and distant lineage.

==> Makefile <==
# Makefile for thesis.
# Simply run `make` to build the thesis.pdf.
# You can also use `make pvc` to "preview continuously" (i.e. pdf will update
# in real time while editing the source files).
# Use `make clean` to remove all generated files.
# Note that all auxilliary files will be stored in the `aux` directory to keep
# the root directory clean.
#
# This is roughly based on: 
# https://drewsilcock.co.uk/using-make-and-latexmk
# http://tex.stackexchange.com/questions/40738/how-to-properly-make-a-latex-project
#

LATEX=xelatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode
AUXDIR=aux

LATEXMK=latexmk
LATEXMKOPT=-pdf -outdir=$(AUXDIR) -auxdir=$(AUXDIR)
CONTINUOUS=-pvc

MAIN=thesis
OUTPUT_FILENAME=thesis
SOURCES := Makefile $(shell find . -regex '.*\.\(tex\|cls\|sty\|bib\)')
ADDITIONAL_FILES := README.md
FIGURES := $(shell find graphics/* -type f)

all: symlink once

once: symlink
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

.refresh:
	touch .refresh

pvc: aux $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

# Create a symlink for the final PDF
symlink: aux
	rm -f $(OUTPUT_FILENAME).pdf
	ln -Fs $(AUXDIR)/$(MAIN).pdf $(OUTPUT_FILENAME).pdf

clean:
	$(LATEXMK) -C $(MAIN) -quiet
	$(shell echo "find . -name '*.aux' -print0 | xargs -0 rm -f")
	$(shell find . -name '*.aux' -print0 | xargs -0 rm -f)
	rm -rf aux
	rm -f .refresh
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.end *.fls *.log *.out *.fdb_latexmk *.cb *.thm
# not removing the biber cache - it's not guaranteed that biber is even available,
# or that biber --cache gives something meaningful

aux:
	mkdir -p aux aux/front aux/back aux/misc aux/main

$(MAIN).zip: $(SOURCES) $(FIGURES) $(ADDITIONAL_FILES)
	rm -f $(MAIN).zip
	zip $(MAIN).zip $(SOURCES) $(FIGURES) $(ADDITIONAL_FILES)

archive: $(MAIN).zip
zip: $(MAIN).zip


.PHONY: clean once symlink all aux


==> algorithms/formula_approx.tex <==
\begin{figure}[h]
\removelatexerror% Nullify \@latex@error
\begin{algorithm2e}[H]
\SetAlgoLined
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \SetKwFunction{ClusterVectorsUsingKMeans}{\fncolor{ClusterVectorsUsingKMeans}}
\SetKwData{pv}{LV$_3$}
% \SetKwInOut{HP}{Hyper-Parameters}

% \HP{\textit{max\_vectors\_num} - maximum number of vectors per-tuple}
\KwIn{two sets of lineage vectors $LV_1, LV_2$ that represent the lineage of two tuples $t_1$ and $t_2$, respectively}
\KwResult{a new set of lineage vectors \pv, that represents $t_1 + t_2$}
\BlankLine
\BlankLine
 \cmtcolor{\tcc{Call this algorithm via $+(LV1,LV2)$ or using the infix notation $LV1 + LV2$}}
 \BlankLine
%  $\pv = LV_1 \cup LV_2$\;
%  \If{$|\pv| > max\_vectors\_num$}{
%     \cmtcolor{\tcc{Perform K-Means clustering over the vectors into \textit{max\_vectors\_num} groups and return the centers (i.e., each center is a vector) of each group}}%\label{cmt}
%     \pv = \ClusterVectorsUsingKMeans{\paramcolor{$\pv$}}\;
%  }
\end{algorithm2e}
\caption{Convert provenance formula to lineage vectors}\label{algo:formula_offline_approx}
\end{figure}

==> algorithms/init_approx_prov.tex <==
% \begin{figure}[h]
\removelatexerror% Nullify \@latex@error
\begin{algorithm2e}
\begin{small}
\SetAlgoLined
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwFunction{WeightedAverage}{\fncolor{WeightedAverage}}
\SetKwData{vt}{v$_t$}

\KwIn{a pre-trained word embeddings model $M$, an input database $D$}
\KwResult{calculate an initial lineage vector \vt for every tuple $t$ in $D$}
\BlankLine
\BlankLine
 \For{$t \in D.tuples$}{
  \cmtcolor{\tcc{$M$ is a pre-trained word embeddings model and $t$ is a DB tuple}}
  $word\_vectors_t = \{M(w)\mid w \in t\}$\;
  \cmtcolor{\tcc{An intra and inter-column weighted average over the vectors of every word in $t$
%   That is, average the word vectors for each column separately, and then apply weighted average on the "column vectors".
  }}%\label{cmt}
  \vt = \WeightedAverage{\paramcolor{$word\_vectors_t$}}\;
}
\caption{Lineage vectors: Initialization Algorithm}\label{algo:init_approx}
\end{small}
\end{algorithm2e}
% \caption{Lineage vectors: Initialization Algorithm}\label{algo:init_approx}
% \end{figure}

==> algorithms/provsql_approx.tex <==
\begin{figure}[h]
\removelatexerror% Nullify \@latex@error
\begin{algorithm2e}[H]
\SetAlgoLined
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \SetKwFunction{ClusterVectorsUsingKMeans}{\fncolor{ClusterVectorsUsingKMeans}}
\SetKwData{token}{token$_3$}
% \SetKwInOut{HP}{Hyper-Parameters}

% \HP{\textit{max\_vectors\_num} - maximum number of vectors per-tuple}
\KwIn{a pair of tokens $token_1, token_2$ 
and their associated sets of lineage vectors $LV_1, LV_2$\newline
an operation $op \in \{+, \cdot\}$}
\KwResult{a new token \token, that is associated with the new set of lineage vectors $LV_3$ = $LV_1\:op\:LV_2$}
\BlankLine
\BlankLine
 \BlankLine
 \Switch{$op$}{
    \Case{$+$}{
        $LV_3$ = $LV_1 + LV_2$ \cmtcolor{\tcp*{see Algorithm \ref{algo:add_approx}}}
    }
    \Case{$\cdot$}{
        $LV_3$ = $LV_1 \cdot LV_2$ \cmtcolor{\tcp*{see Algorithm \ref{algo:mul_approx}}}
    }
 }
 tag the newly generated $LV_3$ as \token\;
\end{algorithm2e}
\caption{Incorporating lineage vectors in the ProvSQL Algorithm}\label{algo:provsql_online_approx}
\end{figure}

==> figures/q1.tex <==
\newcommand{\sqlcolor}[1]{\textcolor{Bittersweet}{#1}}
\newcommand{\fieldcolor}[1]{\textcolor{Fuchsia}{#1}}
\newcommand{\strcolor}[1]{\textcolor{ForestGreen}{#1}}

% \begin{adjustbox}{width=\columnwidth,center}
\begin{figure}[h]
% \raggedright
% \begin{small}
    \texttt{
    % \textcolor{white}{\tiny something}\\
    \textcolor{white}{F}\sqlcolor{SELECT DISTINCT} \fieldcolor{manufacturer} \\
    \textcolor{white}{FF}\sqlcolor{FROM} products p, nutrients n\\
    \textcolor{white}{FF}\sqlcolor{WHERE} p.\fieldcolor{ndb\_no} = n.\fieldcolor{ndb\_no} \\ 
    \textcolor{white}{FF}\sqlcolor{AND} n.\fieldcolor{nutrient\_name} = \strcolor{'cholesterol'}
    }
    % \textbf{\caption{\label{fig:queries_usda_bpfd}Running example query for the USDA Branded Products Food Database}}
% \end{small}
\end{figure}
% \end{adjustbox}

==> main/chap1_classic_prov.tex <==
\section{Classic Provenance}
\label{chap:classic_provenance}

% \subsection{Classic Provenance}

\subsection{Definition}
% Dictionary entry
Provenance - \textit{source, origin} \cite{prov_dict}. 
% General explanation
In computing, provenance information describes the origins and the history of data within its lifetime. When talking about database management systems, the commonly used term is \textit{data provenance} \cite{cheney2009provenance}. The idea behind data provenance is keeping additional information (meta-data) allowing us to easily answer a number of useful ``meta-questions''.
% Provenance as explanations for query results
\par Data provenance helps with providing explanations for the existence of tuples in a query result. The context of these explanations is usually the DB state prior to the query execution.

% Intro to notions of data provenance
\subsection{Related Work}\label{sec:related_work}
Over the past 15 years, provenance research has advanced in addressing both theoretical \cite{cheney2009provenance, green2007provenance, Deutch2014} 
and practical \cite{Ives2008, Karvounarakis2010, Deutch2015, Deutch2017, Senellart2018, DBLP:conf/cidr/IvesZHZ19} 
aspects. 
In particular, several different notions of data provenance (\textit{lineage}, \textit{why}, \textit{how} and \textit{where}) were formally defined \cite{Cui:2000:TLV:357775.357777, DBLP:conf/icdt/BunemanKT01,  cheney2009provenance}.
% Related Work - Provenance Approximation and Summarization
\par A few prior works \cite{approx_lineage, approx_PROX, approx_summary, approx_why_and_why_not} focus on approximate (or summarized) provenance. That is, seeking a compact representation of the provenance, at the possible cost of information loss, in an attempt to deal with the growing size and complexity of exact provenance data in real-life systems.


% \subsection{Provenance Semirings}\label{sec:semiring provenance}
% % Overview and definition - Val Tannen and T.J. Green
% \subsubsection{Overview}\footnotemark
% \footnotetext{Portions of this section were adapted from Green et al. \cite{green2007provenance} and Karvounarakis et al. \cite{Karvounarakis:2012:SDQ:2380776.2380778}.}
% \textit{Provenance semirings} have been introduced by Green et al. \cite{green2007provenance} as a formalism for data provenance. These semirings have been shown \cite{Karvounarakis:2012:SDQ:2380776.2380778} to generalize previous works such as lineage \cite{Cui:2000:TLV:357775.357777} and why-provenance \cite{DBLP:conf/icdt/BunemanKT01}. The main idea is based on annotating (\textit{tagging}) every tuple in the DB with elements from some algebraic structure $(K,+,\cdot,0,1)$\footnotemark
% \footnotetext{$K$ is a set, containing two distinguished elements $0,1$; and $+,\cdot$ are binary operators on elements from $K$.}
% resulting in tagged-tuple relations.
% A notationally convenient way of working with tagged-tuple relations is to model tagging by a function on all possible tuples, with those tuples not considered to be ``in'' the relation tagged with a special value (usually, it is the $0$ element from the set $K$).
% \par Let us denote the set of all tuples over a finite set of attributes $U$ by $U$-Tup.
% A $K$-relation over a finite set of attributes $U$ is a function $R: U$-Tup $\rightarrow K$ such that its support\footnotemark\hspace{0.2mm} is finite.
% \footnotetext{$\operatorname{support}(R) = \{t\;|\;R(t) \neq 0 \}$.}
% The following definitions view an $\mathcal{RA^+}$ (relational algebra, excluding the difference operator) expression $E$ as a $K$-relation, namely a function. The definition is recursive on the structure of $\mathcal{RA^+}$ expression $E$:
% \begin{itemize}
%     \item \textbf{empty relation.} For any set of attributes $U$, there is a function $\emptyset : U$-Tup $ \rightarrow K$ such that $\emptyset(t) = 0$, $\forall t \in U$-Tup.
%     \item \textbf{union.} If $R_1, R_2 : U$-Tup $ \rightarrow K$ then $R_1 \cup R_2 : U$-Tup $ \rightarrow K$ is defined by $(R_1 \cup R_2)(t) \triangleq R_1(t) + R_2(t)$, $\forall t \in U$-Tup.
%     \item \textbf{projection.} If $R : U$-Tup $ \rightarrow K$ and $V \subseteq U$ then $\pi_VR : V$-Tup $ \rightarrow K$ is defined by $(\pi_VR)(t) \triangleq \sum\limits_{t=t'\;on\;V\;and\;R(t') \neq 0}R(t')$, $\forall t \in U$-Tup.\\
%     (here $t=t'\;on\;V$ means $t' \in U$-Tup whose restriction to $V$ is the same as $t$; note also that the sum is finite since $R$ has finite support).
%     \item \textbf{selection.} If $R : U$-Tup $ \rightarrow K$ and the selection predicate \textbf{P} maps each tuple in $U$-Tup to either $0$ or $1$, then $\sigma_\textbf{P}R : U$-Tup $ \rightarrow K$ is defined by $(\sigma_\textbf{P}R)(t) \triangleq R(t) \cdot \textbf{P}(t)$, $\forall t \in U$-Tup.
%     \item \textbf{natural join\footnotemark.} If $R_i : U_i$-Tup $ \rightarrow K$, i=1,2 then $R_1 \bowtie R_2$ is the $K$-relation over $U_1 \cup U_2$ defined by $(R_1 \bowtie R_2)(t) \triangleq R_1(t_1) \cdot R_2(t_2)$, where $t_1=t$ on $U_1$ and $t_2 = t$ on $U_2$, $\forall t \in U_1 \cup U_2$-Tup.
%     \footnotetext{By renaming attributes that appear in both arguments we can use join to compute cartesian product ($\times$), the basic $\mathcal{RA}$ operator.}
%     \item \textbf{renaming.} If $R : U$-Tup $ \rightarrow K$ and $\beta : U \rightarrow U'$ is a bijection then $\rho_\beta R$ is a $K$-relation over $U'$ defined by $(\rho_\beta R)(t) \triangleq R(t \circ \beta)$, $\forall t \in U'$-Tup.
% \end{itemize}
% As defined above, the operations of $\mathcal{RA^+}$ preserve the finiteness of supports, therefore they map $K$-relations to $K$-relations. Hence, the preceding definitions (of making $\mathcal{RA^+}$ to operate on $K$-relations) define an algebra on $K$-relations.
% Green et al. \cite{green2007provenance} showed that the following $\mathcal{RA}$ properties:
% \begin{itemize}
%     \item join and union are both associative and commutative;
%     \item union has identity $\emptyset$;
%     \item join is distributive over union;
%     \item $\sigma_{false}(R) = \emptyset$ and $\sigma_{true}(R) = R$ ($false$ and $true$ are the uniformly false and true predicates, respectively).
% \end{itemize}
% hold for the positive algebra on $K$-relations \textit{iff} $(K,+,\cdot,0,1)$ is a \textit{commutative semiring}.
% I.e., $(K,+,0)$ and $(K,\cdot,1)$ are commutative monoids\footnotemark,
% \footnotetext{An algebraic structure that is closed under an associative binary operation and has an identity element.} 
% $\cdot$ is distributive over + and $\forall a, 0 \cdot a = a \cdot 0 = 0$.

% % Important Cases
% \subsubsection{Important cases} Several important semirings that are discussed in the literature \cite{green2007provenance, Karvounarakis:2012:SDQ:2380776.2380778, Senellart2017} are:
% \begin{itemize}
%     \item $(\mathbb{B}, \vee, \wedge, false, true)$ - binary trust (set semantics, $\mathbb{B} = \{true, false\}$);
%     \item $(\mathbb{N}, +, \cdot, 0, 1)$ - multiplicity (bag semantics, $\mathbb{N}$ is the set of natural numbers);
%     \item $(\mathbb{A}, min, max, 0, P)$ - security semiring (access control), where the total order $\mathbb{A}=P<C<S<T<0$ describes levels of security clearance: $P$ public, $C$ confidential, $S$ secret, and $T$ top-secret;
%     \item $([0,1], max, \cdot, 0, 1)$ - Viterbi semiring (confidence scores, probability);
%     % \item $(\mathbb{N}\cup\{\infty\}, min, +, \infty, 0)$ - tropical semiring (data pricing);
%     \item $(\mathbb{N}[X], 0, 1, +, \cdot)$ - used for a general form of provenance, the provenance polynomials (the universal semiring). $\mathbb{N}[X]$ is the set of multivariate polynomials with coefficients from $\mathbb{N}$ and variables from a set $X$.
% \end{itemize}


% \subsection{Provenance for Data-Dependent Processes}
% % what is a data-dependent process?
% A Data-Dependent Process (DDP) is a logical flow that is specified by a finite state machine (FSM) whose transitions are either governed by boolean queries over an underlying database, or otherwise correspond to external effects such as user choices, interacting applications, etc.
% % Deutch's work
% \par Deutch et al. \cite{Deutch_DDP} suggested approaching the problem of analyzing DDPs using data provenance practices. In particular, in their study, they use provenance semirings \cite{green2007provenance} to obtain a mathematical expression that describes an execution path over the FSM (such a path models a possible execution of a DDP). The transitions on such a path depend on queries over a database or on external user actions. Deutch et al. introduced a new method for generalizing provenance semirings to the context of DDP analysis. This is achieved by using two separate (and potentially, different) semirings - one for user actions and the other for DB tuples, and combining them by a novel \textit{tensor product} construction, as opposed to completely separating the two kinds of provenance semirings by e.g., a simple cartesian product of the two semirings. The proposed method allows to construct a generalized provenance expression (using polynomials) for a possible execution of a DDP and to specialize it using homomorphisms \cite{green2007provenance}.
% \par In terms of methodology, keeping track of provenance of a DDP along an execution path (as long as the path is finite) is intuitively similar to tracking provenance of a query result, where each edge on the path is a piece of data (with its own provenance, e.g., an intermediate result), and the whole path corresponds to a joint use of the pieces of data.
% % comparison to a single-query provenance analysis


% \subsection{ProvSQL - A Real World Provenance Generating Application}\label{sec:provsql}
% Goal
\par ProvSQL is an open-source project developed by Pierre Senellart et al. \cite{Senellart2018}.
According to \cite{provsql_github}:
``The goal of the ProvSQL project is to add support for (m-)semiring provenance and uncertainty management to PostgreSQL databases, in the form of a PostgreSQL extension/module/plugin.''
% and briefly discuss their implementation.
% % m-semirings
% \subsubsection{Semirings with monus} We previously stated in section \ref{sec:semiring provenance} that provenance semirings cover only $\mathcal{RA^+}$ queries. However, \cite{monus_k_relations} identified a large class of semirings that (subject to certain restrictions) can be equipped with a monus operator $-$. Thus, it is possible to generalize provenance capturing to $\mathcal{RA}$ with a difference $(\setminus)$ operation (adding support for non-monotone\footnotemark queries). 
% \footnotetext{Non-monotone means: $I \subseteq I' \notimplies Q(I) \subseteq Q(I')$.}
% This class of semirings is called \textit{m-semirings}. Furthermore, \cite{monus_k_relations} show a universal m-semiring, i.e., it is possible to obtain a provenance evaluation in any other m-semiring by applying an appropriate semiring homomorphism.
% Provenance Circuits
ProvSQL uses \textit{circuits}, a compact representation for provenance annotations \cite{Deutch2014, Senellart2017}, which are constructed per-query. A provenance circuit is an inductively built directed acyclic graph (DAG), with the following properties:
\begin{enumerate*}
    \item The leaves contain annotations of tuples from the input DB.
    \item Inner nodes (termed \textit{gates}) represent operators from a particular semiring. 
    \item The edges (termed \textit{wires}) connect nodes to an operator, representing operands of an intermediate calculation.
    \item The sub-DAG under a given node represents the semiring formula for deriving it. 
\end{enumerate*}
% % PostgreSQL Hooks
% \subsubsection{PostgreSQL Hooks} PostgreSQL (Postgres) hooks \cite{postgre_hooks} make it possible to extend/modify its behaviour without rebuilding Postgres, by interrupting the execution process at certain points. Similarly to Postgres itself, the hooks API is written in C. Every hook is accessible via a global function pointer, initially set to \texttt{NULL}. During an extension's loading (following a \texttt{CREATE EXTENSION} command) Postgres calls the extension's own \texttt{\_PG\_init} function (if implemented), which has access to the hooks handler pointers (at this point, a hook function can be registered). When Postgres needs to call a hook, it checks the relevant function pointer, and calls the registered function, if the pointer is set (i.e., not \texttt{NULL}).
% % Implementation
% \subsubsection{Implementation} ProvSQL \cite{provsql_github} uses the \texttt{planner\_hook}, which is called after a query has been parsed, and before it is sent to the query planner. 
% ProvSQL currently supports a wide range of non-aggregate SQL queries (for more details see \cite{provsql_github, Senellart2018}). The generated query result includes a \texttt{provsql} column of unique\footnotemark
% \footnotetext{128-bit universally unique identifiers (UUIDs) that are generated using the \texttt{uuid-ossp} PostgreSQL module.}
% tokens, identifying gates of the produced provenance circuit.



==> main/chap2_lineage_embeddings.tex <==
\section{Lineage via Embeddings}
\label{chap:lineage_embeddings}

\subsection{Word Embeddings}\label{sec:word_embeddings_intro}
% The need for word embeddings in NLP
Classic NLP research focuses on understanding the structure of text. For example, building dependency-based parse trees \cite{melcuk1988, klein-manning-2004-corpus} that represent the syntactic structure of a sentence via grammatical relations between its words. These approaches do not account for the \textbf{meaning} of words. \textit{Word embedding} aims to encode meanings of words (i.e., semantics), via low dimension (usually, 200-300) real-valued vectors, which can be used to compute the similarity of words as well as test for analogies \cite{DBLP:conf/naacl/MikolovYZ13}. Two of the most influential methods for computing word embeddings are the \textsc{Word2Vec} family of algorithms, by Mikolov et al. \cite{DBLP:journals/corr/abs-1301-3781, DBLP:conf/nips/MikolovSCCD13} and \textsc{GloVe} by Pennington et al. \cite{pennington2014glove}. Furthermore, applying neural-network (NN) techniques to NLP problems (machine translation \cite{wu2016googles}, named entity recognition \cite{Gillick_2016}, sentiment analysis \cite{Maas:2011:LWV:2002472.2002491} etc.) naturally leads to the representation of words and text as real-valued vectors. 

\subsection{Motivation}\label{sec:motivation_approx}
A few problems become apparent when considering \textit{Distant Lineage} (i.e., indirect, history long, explanations for the existence of tuples in the DB) with traditional and state of the art ``exact provenance tracking'' techniques:
\begin{enumerate*}
    \item Formula based representations may \textit{blow-up} in terms of \textit{space consumption}.
    A naive implementation using semiring polynomials \cite{green2007provenance} requires saving the full provenance polynomial for each tuple, resulting in a massive growth in space consumption (for tuples that are produced by a query and that may depend on result tuples of previous queries).
    % That is, a \textit{constant space per-tuple} representation is essential for practical provenance tracking in modern DB systems. 
    
    \item Inductively built representations become very complex over time. Thus, they result in impractical provenance querying time. A naive implementation using circuits \cite{Deutch2014, Senellart2017} would simply keep on constructing provenance circuits as described in section \ref{sec:related_work}. During lineage querying, we may end up with very complex circuits, such that numerous leaves are derived via a circuit of their own (these leaves are tuples that were produced by a previous query and were inserted to the DB). Hence, even if a significant amount of sharing is realized across the provenance circuits - they are inevitably going to blow-up in space consumption. This approach renders keeping and querying the full provenance as impractical and requires limiting heavily the provenance resolution, otherwise (e.g., return a summarized explanation). That is, \textit{querying complex data structures} like circuits is impractical for provenance querying in modern DB systems.
    
    \item Alternatively, if we only want lineage, we could just store with each tuple a set of all the tuples it depends on. This will be cheaper than circuits but still prohibitively expensive. Here too, one could think of circuit-like techniques where tuples that have a subset in common, of tuples in their lineage, could share this subset. But again, this is complex and suffers from similar problems, as discussed above.
    
    \item Complex explanations are not very human-readable. Deutch et al. \cite{Deutch2017} showed how to generate more human-readable explanations - but they are arguably still complex. A ``top-$k$ justifications'' style provenance, which is \textit{simpler} and provides \textit{ranking} of justifications, might be more useful for an analyst in a real-time interaction with the data.
\end{enumerate*}

\par Consider an illustrative example using ProvSQL. Suppose there is a database with two relations: \texttt{Edge(A,B)} - a tuple $(a,b)$ denotes an undirected edge between $a$ and $b$, and \texttt{Path(X,Y)} - a tuple $(x,y)$ denotes a path from node $x$ to node $y$. Suppose that for all $a,b$ that appear in the DB, call them \textit{nodes} and assume there are $\#N$ distinct nodes, \texttt{Edge($a,b$)} exists, i.e., \texttt{Edge} encodes a complete graph. 
Assume $\#E$ is the number of tuples in the \texttt{Edge} table, that is, $\#E = \frac{\#N \cdot (\#N - 1)}{2}$.
Some of the tuples in \texttt{Path} were inserted manually. Others, such as for node 7, were inserted based on the query:
\input{figures/q_space_the_final_frontier}
The result is the tuples \texttt{Path($a,7$)} for all  nodes $a$ in the DB (since the graph is complete, there is a 6-edge length path between every pair of nodes).
Now, the lineage of each such tuple is all the \texttt{Edge} tuples, but the circuit needs to encode the different 6-edge paths separately (it corresponds to a different ordered subset of the set of tuples in \texttt{Edge}, starting with node $a$ and ending with node $7$). For each path from $a$ to $7$, ProvSQL (see section \ref{sec:related_work}) creates a circuit gate encoding the path and 6 wires (for each one of the edges in the path).
There are $(\#N - 2) \cdot (\#N - 3) \cdot (\#N - 4) \cdot (\#N - 5) \cdot (\#N - 6) = O(\#N^5) = O(\#E^{2.5})$
such paths from $a$ to $7$. So, ProvSQL needs to allocate $O(\#E^{2.5})$ gates, each one connected to 7 wires.
In other words, this is very much not linear in the size $O(\#E)$ of the database. Notice that choosing a different query with longer paths only makes matters worse for ProvSQL. On the other hand, the method we present in this paper requires only a constant additional space for each of the query result tuples.

% \section{Proposed Solution}\label{sec:proposed_solution_approx}
% % Our proposal - encode provenance information using word embeddings
% \par We devise a novel approach to provenance tracking, which is based on ML and NLP techniques. The main idea is summarizing, and thereby approximating, the lineage of every tuple with a set of up to $max\_vectors\_num$ (a hyperparameter) vectors. For tuples that are inserted explicitly into the DB, the vectors are obtained using a pre-trained word embeddings model $M$ over the underlying ``text'' of the tuple (see Figure \ref{algo:init_approx}).
% During a query execution process we form the lineage of new query result tuples in a similar fashion to that of provenance semirings \cite{green2007provenance}. We extend the + and $\cdot$ operations (see Figures \ref{algo:add_approx} and
% \ref{algo:mul_approx}, respectively) to generate lineage embeddings, while emphasizing the ability to propagate information and preserve the representation of lineage via a set of up to $max\_vectors\_num$, constant-size vectors. We obtain lineage embeddings for query output tuples by using this process. These new tuples (and their lineage) may be later inserted into the DB (depending on the specific application). 
% \par A real world provenance system like ProvSQL \cite{provsql_github} can make use of our lineage vectors during the construction of provenance circuits. Recall that each node in a provenance circuit is associated with some annotation/token, either representing a tuple from the input DB or an intermediate calculation (see section \ref{sec:provsql}). Lineage vectors can be incorporated in such a system by calling the Algorithm in Figure \ref{algo:provsql_online_approx}, for instance. This is an ``online'' approach, meaning the lineage vectors are generated during the query execution process. Another approach to incorporating lineage vectors in a real world provenance system might be using such a system as a black box, generating a provenance how-formula for each query output tuple. Later, this formula can be analyzed ``offline'', parsed, and converted to lineage vectors by evaluating the parsed expression in a hierarchical manner. Each intermediate evaluation step would call either Figure \ref{algo:add_approx} or \ref{algo:mul_approx}, based on the parsing of the formula, mimicking the online nature of algorithm \ref{algo:provsql_online_approx}.


% \begin{runexample}
%     % Show examples of addition and multiplication constructions
%     Next, we show examples of the addition and multiplication lineage vectors constructions (Figures \ref{algo:add_approx} and
% \ref{algo:mul_approx}, respectively).
%     Let $\vec v_1, \vec v_2, \vec v_3, \vec v_4 \in \mathbb{R}^2$ be vectors, such that:
%     \begin{equation*}
%         \vec v_1 = \begin{pmatrix} -1\\ 0.5 \end{pmatrix},
%         \vec v_2 = \begin{pmatrix} 1\\ 1 \end{pmatrix},
%         \vec v_3 = \begin{pmatrix} -0.5\\ 1 \end{pmatrix},
%         \vec v_4 = \begin{pmatrix} 0\\ -1 \end{pmatrix}
%     \end{equation*}
%     Suppose we have two tuples $t_1, t_2$ with respective sets of lineage vectors $LV_1, LV_2$, such that:
%     \begin{equation*}
%         LV_1 = \{\vec v_1, \vec v_2, \vec v_3\}, LV_2 = \{\vec v_4\}
%     \end{equation*}
%     Finally, the hyperparameters are:
%     \begin{equation*}
%         max\_vectors\_num = 3
%     \end{equation*}
% \end{runexample}
% % addition
% \begin{example-withrun}
%     Let us follow the construction of $LV_3$, which represents the lineage embeddings of $t_1 + t_2$ using the addition Algorithm in Figure \ref{algo:add_approx} (corresponds to alternative use of data, i.e., OR in the query):
%     \begin{enumerate}
%         \item $LV_1 \cup LV_2 = \{\vec v_1, \vec v_2, \vec v_3\} \cup \{\vec v_4\} = \{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}$
%         \item $|\{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}| = 4 > 3 = max\_vectors\_num$
%         \item $LV_3 = \operatorname{ClusterVectorsUsingKMeans}(\{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}) = \{\vec c_1, \vec c_2, \vec c_3\}$\\
%         such that: 
%         \begin{equation*}
%             \vec c_1 = \begin{pmatrix} -0.75\\ 0.75 \end{pmatrix},
%             \vec c_2 = \begin{pmatrix} 1\\ 1 \end{pmatrix},
%             \vec c_3 = \begin{pmatrix} 0\\ -1 \end{pmatrix}
%         \end{equation*}
%         are the centroids of the three clusters.
%     \end{enumerate}
% \end{example-withrun}
% % multiplication
% \begin{example-withrun}
%     Let us follow the construction of $LV_3$, that represents the lineage embeddings of $t_1 \cdot t_2$ using the multiplication Algorithm in Figure \ref{algo:mul_approx} (corresponds to joint use of data, i.e., AND in the query):
%     \begin{enumerate}
%         \item $\operatorname{CartesianProduct}(LV_1, LV_2) = \{(\vec v_1, \vec v_4), (\vec v_2, \vec v_4), (\vec v_3, \vec v_4)\}$
%         \item $\{\operatorname{Avg}(\vec v_1, \vec v_4), \operatorname{Avg}(\vec v_2, \vec v_4), \operatorname{Avg}(\vec v_3, \vec v_4)\} = \{\vec a_1, \vec a_2, \vec a_3\}$\\
%         such that:
%         \begin{equation*}
%             \vec a_1 = \begin{pmatrix} -0.5\\ -0.25 \end{pmatrix},
%             \vec a_2 = \begin{pmatrix} 0.5\\ 0 \end{pmatrix},
%             \vec a_3 = \begin{pmatrix} -0.25\\ 0 \end{pmatrix}
%         \end{equation*}
%         are the average vectors, of each pair, in the cartesian product.
%         \item $|\{\vec a_1, \vec a_2, \vec a_3\}| = 3 \leq 3 = max\_vectors\_num$
%         \item $LV_3 = \{\vec a_1, \vec a_2, \vec a_3\}$
%     \end{enumerate}
% \end{example-withrun}
% % Algorithm - use Algorithm2e
% \input{algorithms/init_approx_prov.tex}
% % \footnotetext{The square brackets notation [ ] constructs a list, analogous to set construction. The order of words in the list is arbitrary.}
% \input{algorithms/add_approx_prov.tex}
% \input{algorithms/mul_approx_prov.tex}
% \input{algorithms/provsql_approx.tex}
% % \input{algorithms/formula_approx.tex}


% % \footnotetext{Perform K-Means clustering over the vectors into \textit{max\_vectors\_num} groups and return the centers of each group.}

% % Explain the motivation and process of approx provenance querying

% \subsection{Lineage querying} As was mentioned in section \ref{sec:word_embeddings_intro}, word embeddings (i.e., vectors) provide insights into the meaning of words via a word-word similarity score. The similarity measure is the cosine distance between the word vectors. Our goal is to construct and maintain lineage embeddings, which can provide insights to the reasons for the existence of tuples via a tuple-tuple similarity score, which is analogous to word-word similarity score (the tuples of interest are the ones generated by a query, which in turn use previously query-generated tuples as well as explicitly inserted ones).
% \par Consequently, given a tuple and its lineage embeddings, we can calculate the pair-wise similarity against every other tuple in the DB (or a subset, e.g., in a specific table) and return the top $k$ (a parameter) most lineage-similar tuples (these resemble a subset of the lineage \cite{Cui:2000:TLV:357775.357777}). 
% There are many algorithms for approximate vector search, e.g., based on LSH \cite{lsh}. Approximate vector search is a very active area of research and we can utilize known algorithms (see, e.g., \cite{sugawara-etal-2016-approximately}).
% Due to the reliance of lineage embeddings on an underlying statistical ML model, we expect our produced lineage to \textbf{approximate} the exact \textbf{lineage}.\\

% % \footnotetext{Call this algorithm via $+(LV1,LV2)$ or using the infix notation $LV1 + LV2$.}
% % \footnotetext{Call this algorithm via $\cdot(LV1,LV2)$ or using the infix notation $LV1 \cdot LV2$.}

% % indtended usage clarification
% \subsection{Intended usage} The intended usage of lineage vectors is as follows:
% \begin{itemize}
%     \item Each manually inserted tuple - has a set consisting of a single tuple vector.
%     \item Each tuple in the result of a query - has a set of up to $max\_vectors\_num$ tuple vectors.
%     \item When calculating similarity - we always compare between two sets of lineage vectors, by using the formula we shall present in section \ref{sec:latent_wv_model}.
% \end{itemize}
% % Show how our approach addresses the problems listed in the motivation section
% \subsection{Comparison to exact lineage} In section \ref{sec:motivation_approx} we listed some problems that arise when approaching distant (i.e., over the whole DB history) lineage computation with traditional techniques. Our proposed solution addresses these problems as follows:
% \begin{itemize}
%     \item Lineage embeddings require only a constant space per-tuple.
%     \item Lineage embeddings are immutable once computed, and do not get more complex over time (querying time depends only on the number of tuples, with which we compare the target tuple, i.e., the one to be explained via lineage).
%     \item Returned explanations (produced lineage) are simply the top-N justifications, and may assist in further analysis.
% \end{itemize}
% We approximate lineage using embedding techniques. As noted, lineage is a type of provenance, and it can be expressed using semirings. Now, semirings can also express how-provenance, which is more general and informative than lineage, but, it becomes extremely complex to track as histories develop. Thus, lineage seems to be a more practical tool for analysts.
% A major advantage of our approach is realized for distant provenance. A process that is equivalent functionally to recursive drill through is done automatically (i.e., if we envision the distant provenance of a tuple as a recursive tree-like structure).\\

% \par After developing the concept of lineage embeddings in isolation, it is essential to test it as part of a real-world implementation. We developed a Python module that adds ``lineage via embeddings'' capabilities to a Postgres DBMS, by integrating our module with the ProvSQL \cite{Senellart2018} extension. The construction of the lineage vectors is based on the algorithms presented above.


\subsection{Word Vectors Model}\label{sec:latent_wv_model}
% All logic and vector training from db code is written in python (detached from ProvSQL, enabling faster development)
The system we propose is based on word vectors models. Such a model is composed of a collection of real-valued vectors, each associated with a relevant DB term. The process of deriving vectors from DB-derived text is called \textit{relational embedding}, which is a very active area of research \cite{10.1145/3318464.3389742, 10.1145/3464509.3464892, arora2020embeddings}.
% Word Vectors Training
\subsubsection{Training word vectors} 
As in Bordawekar et al. \cite{DBLP:journals/corr/BordawekarS16}, we train a \textsc{Word2Vec} model \cite{rehurek_lrec} on a corpus that is extracted from the relevant DB.
The training time of word vectors on a DB extracted corpus depends on the size of the corpus, in terms of number of tokens, and on the dimensionality of the trained vectors. For example, on the very small 8.4 MB BFPDB database that we used for experimentation, the training time was ~400 secs, on an 8-core Intel Xeon 5220R machine (no GPU). Various training benchmarks are reported in \cite{DBLP:journals/corr/abs-1301-3781}.
% For example, analyzing \textsc{Word2Vec}, Mikolov et al. \cite{DBLP:journals/corr/abs-1301-3781} report training times for different benchmarks.
A naive transformation of a DB to unstructured text (a sequence of sentences) can be achieved by simply concatenating the textual representation of the different columns of each tuple into a separate sentence. This approach has several problems \cite{DBLP:journals/corr/BordawekarS16}.
% \begin{enumerate*}
First, when dealing with natural language text, there is an implicit assumption that the semantic influence of a word on a nearby word is inversely proportional to the distance between them. However, not only that a sentence extracted from a tuple does not necessarily correspond to any natural language structure, but, it can be actually thought of as ``a bag of columns''; i.e., the order between different columns in a sentence has no semantic implications.
Additionally, all columns are not the same. That is, some columns-derived terms may hold more semantic importance than others in the same sentence (generated from a tuple). For instance, a primary key column, a foreign key column, or an important domain-specific column (e.g., a manufacturer column in a products table). This implies that in order to derive meaningful embeddings from the trained word vectors, we need to consider inter-column discrimination, during both word vectors training and lineage vectors construction phases.
% \end{enumerate*}
% \par We solve these problems by properly setting hyperparameters (e.g., window size), artificially (and carefully) injecting repeated text inside a sentence, and dividing the training into multiple, different stages. 
% A detailed outline of the ``textification'' and training processes follows:
% \begin{enumerate*}
%     \item Generate a \texttt{Key} column with unique values for each table in the DB.
%     \item Extract two corpora from the DB, one with columns (except the \texttt{Key} columns) as sentences, and the other with tuples as sentences.
%     \item Transform each numerical value in the generated corpora by concatenating the relevant column name to the number. Other methods of dealing with numerical values exist as well, and are discussed in section \ref{sec:relational_embedding}.
%     \item Transform each sentence in the generated corpora by injecting the corresponding \texttt{Key} value repeatedly after every $k$ (a separate hyperparameter for the columns corpus and the tuples corpus) words in the sentence. The idea is to encode more information about each tuple in its corresponding \texttt{Key} value vector.
%     \item Incrementally train a \textsc{Word2Vec} model on the generated corpora. First, train on the columns corpus and then on the tuples corpus. One may question why we have the same model for both the tuple-based (see section \ref{chap:per_tuple_lineage_vectors}) and the column-based (see section \ref{chap:per_column_lineage_vectors}) lineage vectors. The answer is that experimentally the models that are restricted to only the tuples corpus or only the columns corpus yield inferior results.
% \end{enumerate*}
% One more interesting caveat, of dealing with texts extracted from relations, is that missing data (empty/null cells) is sometimes automatically converted (when an external tool, e.g., Python, is used to interface with PostgreSQL) to `None'. Given that `None' is not a \textit{stop word} (words that are removed from a corpus as part of a common practice of cleanup before training), we realized that `None' adds noise to the vectors (if there is a lot of missing data in the DB). Adding `None' to the list of \textsc{Word2Vec} stop words improved drastically both the word embedding model quality and the overall accuracy of our system.

\par The quality of the word vectors model is crucial to the success of our system. However, optimizing the overall performance should focus not only on the training phase, but also on the way we utilize the trained model. Next, we show one such optimization.
% sentence embeddings
\subsubsection{Sentence embeddings}\label{sec:sentence_embeddings} Extracting sentence embeddings from text has been a well-researched topic in the NLP community over the last seven years. State-of-the-art pre-trained models (e.g., Universal Sentence Encoder \cite{Cer2018UniversalSE, use_github} and BERT \cite{devlin2018bert}) are trained on natural language texts, and thus are not suitable for sentences generated from relational tuples (see discussion above). Hence we train a word embedding model and infer the sentence vectors as a \textit{function of the set of word vectors containing all the words} in a sentence. We average the word vectors for each column separately, and then apply weighted average on the ``column vectors'' (the weight is based on the relative importance of a column, as discussed above). As will be shown, column-based vectors result in significant improvements to lineage encoding.
% % comparing two sets of vectors
% \subsubsection{Similarity calculation}\label{sec:similarity_calculation} Given two word vectors, the similarity score is usually the cosine distance between them. In our system, we want to calculate the similarity between the lineage representations of two tuples/columns (see sections \ref{chap:per_tuple_lineage_vectors} and \ref{chap:per_column_lineage_vectors}, respectively); in both cases, the tuple or column, is associated with a \textit{set} of lineage vectors. That is, we need to calculate the similarity between \textit{two sets of vectors}\footnotemark. The ``logic'' behind the following formula is balancing between the ``best pair'' of vectors (in terms of similarity) in the two sets and the similarity between their average vectors:\\
% \begin{equation*}
%     \operatorname{sim}(A, B) = \frac{w_{max} \cdot max(ps) + w_{avg} \cdot avg(ps)}
%     {w_{max} + w_{avg}}\\
% \end{equation*}
% \footnotetext{We note that \cite{
% DBLP:journals/corr/BordawekarS16, 
% DBLP:journals/corr/abs-1712-07199,
% DBLP:conf/sigmod/BordawekarS17}
% have also used various similar methods for measuring similarity between two sets of vectors.}
% where $ps$ is the set of pair-wise similarities between a pair of vectors, one taken from set $A$ and one taken from set $B$. $w_{max}$ and $w_{avg}$ are (user-specified) hyperparameters. $max$ and $avg$ are functions that return the maximum and average values of a collection of numbers, respectively\footnotemark.
% \footnotetext{This logic holds for both tuple-based vectors and column-based vectors (i.e., for each column separately).}


% \subsection{Related Work}\label{sec:relational_embedding}
% % Relational Embeddings
% \textbf{Relational embedding} is a very active area of research \cite{10.1145/3318464.3389742, 10.1145/3464509.3464892, arora2020embeddings}.
% When converting a relational DB to unstructured text (see section \ref{sec:latent_wv_model}) special care is required to support numerical values correctly. Bordawekar and Shmueli \cite{DBLP:journals/corr/BordawekarS16} take the route of tokenizing numerical values from the DB by preceding each number with a ``range designator'' (e.g., 1-10, 50-100, SMALL, BIG, etc.) in the generated corpus. In \cite{DBLP:journals/corr/abs-1712-07199} Bordawekar, Bandyopadhyay and Shmueli use clustering techniques to represent numerical values textually. In contrast, in this work we deal with numerical values by concatenating the relevant column name to each number in the generated corpus. This way, we ensure our model separates between numerical values of different fields, as they are conceptually different, semantically speaking (for example, we want the value 300 for a \texttt{nutrient\_code} field in a \texttt{nutrients} table to have a different learned vector than the value 300 for a \texttt{household\_serving\_size} field in a \texttt{serving\_size} table, from the USDA BFPDB \cite{usda_bfpd-dataset} dataset). In the specific database example with which we experimented, this simple technique proved sufficient.


% \section{Interim Findings and Hurdles}
% We conducted a series of experiments (see chapter \ref{chap:experimental_evaluation}) and came to the following interim conclusions:
% \begin{itemize}
%     \item Our explanations encode the text and not the tuples. Thus, relations with many similar tuples (text-wise) result in our system performing poorly. We assume that most of the problems listed below are symptoms of the same root cause.
%     \item Analysis of direct provenance (i.e., \textit{direct} explanations for the existence of tuples in a query result in terms of existing DB tuples, regardless of their historical raison d'être) on simple, complex (ones that might involve multiple tables with non-trivial joins and non-trivial ``where'' conditions) and composite (that contain sub-queries) queries gives good results ($> 90\%$ accuracy for ``top $50\%$'' of the tuples in the lineage) generally. However, results suffer from inconsistencies sometimes, identifying tuples incorrectly as part of the linaege due to thier textual similarity to actual lineage tuples.
%     \item Distant provenance provides useful results. However, it suffers from the same problem of textual closeness.
% \end{itemize}

% \par In the next chapter we introduce methods that are designed to overcome these defficiencies.

==> main/chap3_per_tuple_lineage_vectors.tex <==
\section{TV - Per-Tuple Lineage Vectors}
\label{chap:per_tuple_lineage_vectors}

\subsection{Proposed Solution}\label{sec:proposed_solution_approx}
% Our proposal - encode provenance information using word embeddings
\par We devise a novel approach to lineage tracking, which is based on ML and NLP techniques. The main idea is summarizing, and thereby approximating, the lineage of every tuple with a set of up to $max\_vectors$ (a hyperparameter) vectors. For tuples that are inserted explicitly into the DB, the vectors are obtained using a pre-trained word embeddings model $M$ over the underlying ``text'' of the tuple $t$, applying an intra and inter-column weighted average over the vectors of every word in $t$.
During a query execution process we form the lineage of query result tuples in a similar fashion to that of provenance semirings \cite{green2007provenance}. We extend the + and $\cdot$ operations (see Algorithms \ref{algo:add_approx} and
\ref{algo:mul_approx}, respectively) to generate lineage embeddings, while retaining the ability to propagate information and preserve the representation of lineage via a set of up to $max\_vectors$, constant-size vectors. We obtain lineage embeddings (i.e., vectors) for query output tuples by using this process. These new tuples (and their lineage) may be later inserted into the DB (depending on the specific application).
% BACKUP BACKUP BACKUP
% \par A real world provenance system like ProvSQL \cite{provsql_github} can make use of our lineage vectors during the construction of provenance circuits. Recall that each node in a provenance circuit is associated with some annotation/token, either representing a tuple from the input DB or an intermediate calculation (see section \ref{sec:provsql}). Lineage vectors can be incorporated into such a system by calling the Algorithm in Figure \ref{algo:provsql_online_approx}, for instance. This is an ``online'' approach, meaning the lineage vectors are generated during the query execution process. Another approach to incorporating lineage vectors in a real world provenance system might be using such a system as a black box, generating a provenance how-formula for each query output tuple. Later, this formula can be analyzed ``offline'', parsed, and converted to lineage vectors by evaluating the parsed expression in a hierarchical manner. Each intermediate evaluation step would call either Figure \ref{algo:add_approx} or \ref{algo:mul_approx}, based on the parsing of the formula, mimicking the online nature of algorithm \ref{algo:provsql_online_approx}.


% \begin{runexample}
%     % Show examples of addition and multiplication constructions
%     Next, we show examples of the addition and multiplication lineage vectors constructions (Algorithms \ref{algo:add_approx} and
% \ref{algo:mul_approx}, respectively).
%     Let $\vec v_1, \vec v_2, \vec v_3, \vec v_4 \in \mathbb{R}^2$ be vectors, such that:
%     \begin{equation*}
%         \vec v_1 = \begin{pmatrix} -1\\ 0.5 \end{pmatrix},
%         \vec v_2 = \begin{pmatrix} 1\\ 1 \end{pmatrix},
%         \vec v_3 = \begin{pmatrix} -0.5\\ 1 \end{pmatrix},
%         \vec v_4 = \begin{pmatrix} 0\\ -1 \end{pmatrix}
%     \end{equation*}
%     Suppose we have two tuples $t_1, t_2$ with respective sets of lineage vectors $LV_1, LV_2$, such that:
%     \begin{equation*}
%         LV_1 = \{\vec v_1, \vec v_2, \vec v_3\}, LV_2 = \{\vec v_4\}
%     \end{equation*}
%     Finally, the hyperparameters are:
%     \begin{equation*}
%         max\_vectors = 3
%     \end{equation*}
% \end{runexample}
% % addition
% \begin{example-withrun}
%     Let us follow the construction of $LV_3$, which represents the lineage embeddings of $t_1 + t_2$ using Algorithm \ref{algo:add_approx} (corresponds to alternative use of data, i.e., OR in the query):
%     \begin{enumerate}
%         \item $LV_1 \cup LV_2 = \{\vec v_1, \vec v_2, \vec v_3\} \cup \{\vec v_4\} = \{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}$
%         \item $|\{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}| = 4 > 3 = max\_vectors$
%         \item $LV_3 = \operatorname{ClusterVectorsUsingKMeans}(\{\vec v_1, \vec v_2, \vec v_3, \vec v_4\}) = \{\vec c_1, \vec c_2, \vec c_3\}$\\
%         such that: 
%         \begin{equation*}
%             \vec c_1 = \begin{pmatrix} -0.75\\ 0.75 \end{pmatrix},
%             \vec c_2 = \begin{pmatrix} 1\\ 1 \end{pmatrix},
%             \vec c_3 = \begin{pmatrix} 0\\ -1 \end{pmatrix}
%         \end{equation*}
%         are the centroids of the three clusters.
%     \end{enumerate}
% \end{example-withrun}
% % multiplication
% \begin{example-withrun}
%     Let us follow the construction of $LV_3$, that represents the lineage embeddings of $t_1 \cdot t_2$ using Algorithm \ref{algo:mul_approx} (corresponds to joint use of data, i.e., AND in the query):
%     \begin{enumerate}
%         \item $\operatorname{CartesianProduct}(LV_1, LV_2) = \{(\vec v_1, \vec v_4), (\vec v_2, \vec v_4), (\vec v_3, \vec v_4)\}$
%         \item $\{\operatorname{Avg}(\vec v_1, \vec v_4), \operatorname{Avg}(\vec v_2, \vec v_4), \operatorname{Avg}(\vec v_3, \vec v_4)\} = \{\vec a_1, \vec a_2, \vec a_3\}$\\
%         such that:
%         \begin{equation*}
%             \vec a_1 = \begin{pmatrix} -0.5\\ -0.25 \end{pmatrix},
%             \vec a_2 = \begin{pmatrix} 0.5\\ 0 \end{pmatrix},
%             \vec a_3 = \begin{pmatrix} -0.25\\ 0 \end{pmatrix}
%         \end{equation*}
%         are the average vectors, of each pair, in the cartesian product.
%         \item $|\{\vec a_1, \vec a_2, \vec a_3\}| = 3 \leq 3 = max\_vectors$
%         \item $LV_3 = \{\vec a_1, \vec a_2, \vec a_3\}$
%     \end{enumerate}
% \end{example-withrun}
% Algorithm - use Algorithm2e
% \input{algorithms/init_approx_prov.tex}
\input{algorithms/add_approx_prov.tex}
\input{algorithms/mul_approx_prov.tex}
% BACKUP
% \input{algorithms/provsql_approx.tex}
% \input{algorithms/formula_approx.tex}


% \footnotetext{Perform K-Means clustering over the vectors into \textit{max\_vectors} groups and return the centers of each group.}

% comparing two sets of vectors
\subsubsection{Similarity calculation}\label{sec:similarity_calculation} Given two word vectors, the similarity score is usually the cosine distance between them. In our system, we want to calculate the similarity between the lineage representations of two tuples/columns (see sections \ref{chap:per_tuple_lineage_vectors} and \ref{chap:per_column_lineage_vectors}, respectively); in both cases, the tuple or column, is associated with a \textit{set} of lineage vectors. That is, we need to calculate the similarity between \textit{two sets of vectors}\footnotemark. The ``logic'' behind the following formula is balancing between the ``best pair'' of vectors (in terms of similarity) in the two sets and the similarity between their average vectors:
\begin{equation*}
    \operatorname{sim}(A, B) = \frac{w_{max} \cdot max(ps) + w_{avg} \cdot avg(ps)}
    {w_{max} + w_{avg}}
\end{equation*}
\footnotetext{We note that \cite{DBLP:journals/corr/BordawekarS16, DBLP:journals/corr/abs-1712-07199, DBLP:conf/sigmod/BordawekarS17} have also used various similar methods for measuring similarity between two sets of vectors.}where $ps$ is the set of pair-wise cosine distances between a pair of vectors, one taken from set $A$ and one taken from set $B$. $w_{max}$ and $w_{avg}$ are (user-specified) hyperparameters. $max$ and $avg$ are functions that return the maximum and average values of a collection of numbers, respectively\footnotemark.
\footnotetext{This logic holds for both tuple-based vectors and column-based vectors (i.e., for each column separately).}

% Explain the motivation and process of approx provenance querying

\subsubsection{Lineage querying} 
% BACKUP BACKUP BACKUP
% As was mentioned in section \ref{sec:word_embeddings_intro}, word embeddings (i.e., vectors) provide insights into the meaning of words via a word-word similarity score. The similarity measure is the cosine distance between the word vectors. Our goal is to construct and maintain lineage embeddings, which can provide insights to the reasons for the existence of tuples via a tuple-tuple similarity score, which is analogous to word-word similarity score; the tuples of interest are the ones generated by a query, which in turn use previously query-generated tuples as well as explicitly inserted ones.
% \par Consequently, g
Given a tuple and its lineage embedding vectors, we can calculate the pair-wise similarity against every other tuple in the DB (or a subset, e.g., in a specific table) and return the top $k$ (a parameter) most lineage-similar tuples (these resemble a subset of the lineage \cite{Cui:2000:TLV:357775.357777}). 
There are many algorithms for approximate vector search, e.g., based on LSH \cite{lsh}. Approximate vector search is a very active area of research (see, e.g., \cite{sugawara-etal-2016-approximately}); however, these algorithms are not directly applicable to our method, since we operate on sets of vectors instead of single vectors. We recently devised a method \cite{leybovich2021efficient} that efficiently reduces the set-set similarity problem to vector-vector similarity. This enables using any approximate vector similarity search algorithm to, given a set of vectors, \textit{efficiently} search among sets of vectors for the closest one or $k$-closest ones.
% Due to the reliance of lineage embeddings on an underlying statistical ML model, we expect our produced lineage to \textbf{approximate} the exact \textbf{lineage}.

% \footnotetext{Call this algorithm via $+(LV1,LV2)$ or using the infix notation $LV1 + LV2$.}
% \footnotetext{Call this algorithm via $\cdot(LV1,LV2)$ or using the infix notation $LV1 \cdot LV2$.}

% indtended usage clarification
\subsubsection{Intended usage} The intended usage of lineage vectors is as follows:
\begin{enumerate*}
    \item Each manually inserted tuple - has a set consisting of a single tuple vector.
    \item Each tuple in the result of a query - has a set of up to $max\_vectors$ tuple vectors.
    \item When calculating similarity - we always compare between two sets of lineage vectors, by using the formula for $\operatorname{sim}(A, B)$ of section \ref{sec:similarity_calculation}.
\end{enumerate*}
% Show how our approach addresses the problems listed in the motivation section
% BACKUP BACKUP BACKUP
% \subsubsection{Comparison to exact lineage} In section \ref{sec:motivation_approx} we listed some problems that arise when approaching distant (i.e., over the whole DB history) lineage computation with traditional techniques. Our proposed solution addresses these problems as follows:
% \begin{itemize}
%     \item Lineage embeddings require only a constant space per-tuple.
%     \item Lineage embeddings are immutable once computed\footnotemark, and do not become more complex over time (querying time depends only on the number of tuples, with which we compare the target tuple, i.e., the one to be explained via lineage).
%     \footnotetext{This is the case when the text characteristics of the DB-extracted text are stable. The case of a changing text characteristics is left for future research.}
%     \item Returned explanations (produced lineage) are simply the top-$k$ justifications, and may assist in further analysis.
% \end{itemize}
% We approximate lineage using embedding techniques. As noted, lineage is a type of provenance, and it can be expressed using semirings. Now, semirings can also express how-provenance, which is more general and informative than lineage, but, it becomes extremely complex to track as histories develop. Thus, lineage seems to be a more practical tool for analysts.
% A major advantage of our approach is realized for distant provenance. A process that is equivalent functionally to recursive drill through is done automatically (i.e., if we envision the distant provenance of a tuple as a recursive tree-like structure).\\

% \subsection{Verifying The Lineage}
% Given a method that approximates the top-$k$ justifications for the existence of a query result tuple, as the one presented above, we propose a simple technique to verify the collection of lineage candidates. The idea is applying the query $q$ that generated the tuple to be explained, $t$ to the collection of lineage tuples obtained by our system. If $t$ is output in the result of applying $q$ on these lineage candidates, then we found a sufficiently small (though, non-precise) explanation for $t$. Furthermore, one could utilize an exact provenance tracking application, e.g., ProvSQL \cite{provsql_github} by applying $q$ to the collection of tuples obtained by our system, to explain $t$ (given that $t$ is ``verified''). This technique relies on the fact that executing $q$ on a small collection of tuples (even with exact provenance tracking) is significantly cheaper than applying the query on the whole, potentially large DB.

% \subsection{Interim Findings and Hurdles}
% After developing the concept of lineage embeddings in isolation, it is essential to test it as part of a real-world implementation. We developed a Python module that adds ``lineage via embeddings'' capabilities to a Postgres DBMS, by integrating our module with the ProvSQL \cite{Senellart2018} extension. The construction of the lineage vectors is based on the algorithms presented above.
% \par We conducted a series of experiments (see section \ref{chap:experimental_evaluation}) and came to the following interim conclusions:
% \begin{itemize}
%     \item Our explanations (returned tuples comprising our lineage approximation) encode the DB-resident text and not the tuples. Thus, relations with many similar tuples (text-wise) result in our system performing poorly. We conjecture that most of the problems listed below are symptoms of the same root cause.
%     \item Analysis of direct lineage (i.e., \textit{direct} explanations for the existence of tuples in a query result in terms of existing DB tuples, regardless of their historical raison d'être) on simple, complex (ones that might involve multiple tables with non-trivial joins and non-trivial ``where'' conditions) and composite (that contain sub-queries) queries gives good results ($> 90\%$ accuracy for ``top $50\%$'' of the tuples in the lineage) generally. However, results suffer from inconsistencies sometimes, identifying tuples incorrectly as part of the lineage due to their textual similarity to actual lineage tuples.
%     \item Distant lineage provides useful results. However, it suffers from the same problem (as identified above) of textual closeness.
% \end{itemize}

% \par In the next sections we introduce methods that are designed to overcome these deficiencies.
\subsection{Verifying the Lineage}
Given a method that approximates the top-$k$ justifications for the existence of a query result tuple, as the one presented above, there is a simple technique to partially verify the collection of lineage candidates. The idea is applying the query $q$ that generated the tuple to be explained, $t$, to the collection of lineage tuples obtained by our system. If $t$ is output in the result of applying $q$ on these lineage candidates, then we found a sufficiently small (though, non-precise) explanation for $t$. Furthermore, one could utilize an exact provenance tracking application, e.g., ProvSQL \cite{provsql_github} by applying $q$ to the collection of tuples obtained by our technique, to explain $t$ (given that $t$ is ``verified''). This technique relies on the fact that executing $q$ on a small collection of tuples (even with exact provenance tracking) is significantly cheaper than applying the query on the whole, potentially large, DB. In case the computed lineage is insufficient, it may be extended (adjusting parameters).


\subsection{System Life Cycle}
\input{figures/system_life_cycle}
The chronological life cycle of the system is presented in Figure \ref{fig:system_life_cycle}.
First, a word vectors model $M$ is trained on the DB extracted text (and perhaps other texts, obtained from external sources), as detailed in section \ref{sec:latent_wv_model}. Optionally, the trained model may be combined with an external pre-trained model. 
Next, given an initial state of the DB, a set $V_t$ containing a single vector is obtained for each tuple $t$, using the word vectors model $M$ over the underlying text of $t$. $V_t$ is inserted into an efficient vector set search structure \cite{leybovich2021efficient}. Later, explicitly inserted (non-computed) tuples adhere to the same behaviour.
During ongoing operation, vector sets are computed for query results, following the query execution steps (as described in section \ref{sec:proposed_solution_approx}). Similarly, computed vector sets for newly inserted computed tuples may be later inserted into the efficient vector set search structure.
An analyst may use the lineage vector sets to explore the direct/distant lineage of previously inserted computed tuples or current query results.

==> main/chap4_per_column_lineage_vectors.tex <==
\section{CV - Per-Column Lineage Vectors}
\label{chap:per_column_lineage_vectors}


% \section{Per-Column Lineage Vectors}\label{sec:column-vectors}
\subsection{Rationale} As noted, text obtained from database relations does not behave like natural language text, and a sequence of columns values in a tuple does not usually construct a natural language sentence. Thus, building lineage vectors at the tuple level and comparing tuples on this basis is noisy and potentially lossy in terms of information. Instead, we devise a genetics-inspired approach. Suppose a DB tuple presents the external appearance (i.e., phenotype) of a DB entity, as dictated by the genetic code of the entity. The columns of an entity are its basic properties, i.e., the genes that combine to construct its genetic code. In this setting, querying the direct lineage of a result tuple is analogous to finding its predecessors through DNA tracking. Following the approach presented above, we design an alternative lineage tracking mechanism, that of keeping track of and querying lineage (via embeddings) at the column (gene) level. This way, we manage to better distinguish between the provenance features and the textual characteristics of a tuple.
The rationale behind this method is partially inspired by the construction of ``tuple vectors'' by means of averaging the ``sentence vectors'' of the columns (as discussed in section \ref{sec:sentence_embeddings}).

\subsection{Implementation}\label{sec:cv-implementation}
\begin{enumerate}
    \item Each tuple has a set of (up to \textit{max\_vectors}) \textit{column lineage vectors} per-column, instead of a single set of tuple vectors (per-tuple). Let us denote the set of columns (features, characteristics) for which a tuple $t$ has lineage embeddings as $t.lineage\_columns$.
    \item From now on, we formally denote a column name, using the \textit{full name} notation, as $T.\texttt{Attr}$, such that $T$ is a relation name and \texttt{Attr} is a column name. This is meant to achieve better distinction at the lineage vectors level between tuples that originate from different relations with the same column names. 
    \item Given a tuple $t$, we say that $t.lineage\_columns = $
        \begin{equation*}
            t.native\_columns \cup t.inherited\_columns,
        \end{equation*}
    such that $t.native\_columns$ is the set of data columns of $t$ and $t.inherited\_columns$ is the set of columns (features, characteristics) that $t$ ``inherited'' from its predecessors, but are not necessarily reflected as data columns in $t$.
    Note that the same column name may be in $t$ and inherited from its predecessors as well. This issue will be dealt with shortly.
    In the following examples we use \texttt{A}, \texttt{B}, \texttt{C}, \texttt{D} to represent the full name of a column for brevity. For example, suppose a tuple $t \in T_{AB}$ (a table with only two columns - \texttt{A} and \texttt{B}) has the per-column lineage vectors $CV_t = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_B,\: \texttt{C}\!: LV_C,\: \texttt{D}\!: LV_D\}$ ($CV_t$ is a map of: \textit{$t.lineage\_columns$ $\rightarrow$ sets of lineage vectors}). We say that $t.native\_columns$ = $\{\texttt{A}, \texttt{B}\}$, $t.inherited\_columns$ = $\{\texttt{C}, \texttt{D}\}$ and $t.lineage\_columns$ = $\{\texttt{A}, \texttt{B}, \texttt{C}, \texttt{D}\}$.
    \par\textbf{Note.} From here on, we use the notation $CV_t.columns$ to denote the set of columns in the domain of the map $CV_t$.
    \item When combining lineage embeddings (see Algorithms \ref{algo:add_col_approx},\ref{algo:mul_col_approx}), all calculations are done at the column level.
    \input{algorithms/add_col_approx_prov.tex}
    \input{algorithms/mul_col_approx_prov.tex}
    \item After constructing a new tuple $t \in T$ via a query $q$ and its per-column lineage vectors $CV_t$ (via a series of + and $\cdot$ operations, see Algorithms \ref{algo:add_col_approx} and \ref{algo:mul_col_approx}, respectively) - special care must be taken in constructing lineage vectors per the $native\_columns$ of $t$, which might or might not be inherited from $t$'s predecessors.
    That is, for every column $\texttt{A} \in t.native\_columns$ (\texttt{A} represents the full name of a column for brevity):
    % and $\texttt{A} \notin CV_t.columns$ (after either Algorithm \ref{algo:add_col_approx} or \ref{algo:mul_col_approx} was applied at the last step of constructing $CV_t$)
    \begin{enumerate}
        \item If $\texttt{A} \notin t.inherited\_columns$ and $t.\texttt{A}$ is set to an existing value from some column $\texttt{A'}$ in the DB, e.g., $q$ = \texttt{(INSERT INTO T SELECT A' FROM ...)} then we set $CV_t[\texttt{A}] = CV_t[\texttt{A'}]$.
        \item If $\texttt{A} \in t.inherited\_columns$ and $t.\texttt{A}$ is set to an existing value from some column $\texttt{A'} \neq \texttt{A}$ in the DB, e.g., $q$ = \texttt{(INSERT INTO T SELECT A' FROM ...)} then we set $CV_t[\texttt{A}] =$ $CV_t[\texttt{A}]\; \cdot \;CV_t[\texttt{A'}]$.
        This way, we incorporate both the existing lineage data and the newly calculated one for the column \texttt{A}.
        \item If $\texttt{A} \notin t.inherited\_columns$ and $t.\texttt{A}$ is set to some constant value, e.g., $q$ = \texttt{(INSERT INTO T SELECT \textit{const} FROM ...)} then we set $CV_t[\texttt{A}] = \{initial\_vector(const)\}$, such that $initial\_vector(const)$ is calculated using the pre-trained word vectors model $M$, as described in section  \ref{sec:proposed_solution_approx}, with the ``textified'' (see section \ref{sec:latent_wv_model}) form of \textit{const} as input data.
        \item If $\texttt{A} \in t.inherited\_columns$ and $t.\texttt{A}$ is set to some constant value, e.g., $q$ = \texttt{(INSERT INTO T SELECT \textit{const} FROM ...)} then we set $CV_t[\texttt{A}] = CV_t[\texttt{A}]\; \cdot \; \{initial\_$ $vector(const)\}$. This way, we incorporate both the existing lineage data and the newly calculated one for the column \texttt{A}.
    \end{enumerate}
    % \footnotetext{In the following examples we use the notation \texttt{A}, \texttt{B}, \texttt{C}, \texttt{D} to represent the full name of a column for brevity.}
    % For example, if $t_1$ has lineage vectors for columns \texttt{A},\texttt{B} and $t_2$ has lineage vectors for the columns \texttt{B},\texttt{C} then $t_1 + t_2$ will have lineage vectors $t_1.\texttt{A}$, $(t_1.\texttt{B} + t_2.\texttt{B})$\footnotemark, $t_2.\texttt{C}$ for the columns \texttt{A},\texttt{B},\texttt{C}, respectively. 
    \item When comparing a tuple $t$ (and its lineage embeddings) to a set of other tuples $T'$:
    \begin{enumerate}
        \item If $t'.lineage\_columns \nsubseteq t.lineage\_columns$ ($t' \in T'$) then $t'$ is definitely not a part of the lineage of $t$. Otherwise, all of the ``genes'' (columns) of $t'$ would be reflected in $t$. \label{subsubsec:lineage-columns-filtering}
        \item Ideally, we would have kept all the genes that are affecting the target tuple $t$. However, because of practical reasons (see discussion in \ref{sec:cv_discussion}), sometimes certain genes are dropped.
        Hence, the similarity between $t$ and $t' \in T'$ is averaged over the pair-wise similarities of their respective mutual genes (lineage columns). Notice that without dropping lineage columns, the genes of a potential ancestor $t'$ must be a subset of the genes of $t$.
        For example, say a tuple $t$ that has lineage vectors for columns \texttt{A},\texttt{B},\texttt{C} is compared to another tuple $t'$ that has lineage vectors for columns \texttt{B},\texttt{C},\texttt{D} (here, $t'$ is an arbitrary tuple, which is not necessarily in the lineage of $t$):
        \begin{equation*}
            \operatorname{sim}(t, t') = avg(\{\operatorname{sim}(t.\texttt{B}, t'.\texttt{B}), 
            \operatorname{sim}(t.\texttt{C}, t'.\texttt{C})\})
        \end{equation*}
        where $avg$ is a function that returns the average of a collection of numbers. $\operatorname{sim}(t.\texttt{B}, t'.\texttt{B})$ is the calculated similarity between the lineage vectors for column \texttt{B} of $t$ and $t'$ (similarly for column \texttt{C}). Observe that \texttt{A} and \texttt{D} are not mutual ``genes'' of the tuples $t$ and $t'$, and, thus they do not hold lineage information that is valuable to the similarity calculation.
    \end{enumerate}

\end{enumerate}
% \footnotetext{Here, $(t_1.\texttt{B} + t_2.\texttt{B})$ means applying Algorithm \ref{algo:add_approx} on the respective column lineage vectors.}


\begin{runexample}
    % Show examples of addition and multiplication constructions
    Next, we show examples of the addition and multiplication column lineage vectors constructions (Algorithms \ref{algo:add_col_approx} and \ref{algo:mul_col_approx}, respectively).
    Suppose we have two tuples $t_1, t_2$ with respective maps of \textit{columns $\rightarrow$ sets of lineage vectors} $CV_1, CV_2$, such that:
    \begin{equation*}
        CV_1 = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_{B_1}\},\: CV_2 = \{\texttt{B}\!: LV_{B_2},\: \texttt{C}\!: LV_C\}
    \end{equation*}
    $\texttt{A}, \texttt{B}, \texttt{C}$ are full column names and $LV_A, LV_{B_1}, LV_{B_2}, LV_C$ are sets of lineage vectors.
\end{runexample}
% addition
\begin{example-withrun}\label{example:algo_add_col}
    Let us follow the construction of $CV_3$, which represents the column lineage embeddings of $t_1 + t_2$ using Algorithm \ref{algo:add_col_approx} (corresponds to alternative use of data, i.e., OR in the query):
    \begin{enumerate}
        \item $CV_3 = \{\} \rightarrow \{\}$
        \item $CV_1.columns \,\cup\, CV_2.columns = \{\texttt{A}, \texttt{B}\} \cup \{\texttt{B}, \texttt{C}\} = \{\texttt{A}, \texttt{B}, \texttt{C}\}$
        \item $\texttt{A} \in CV_1.columns \wedge \texttt{A} \notin CV_2.columns $\\ $\Rightarrow CV_3[\texttt{A}] = CV_1[\texttt{A}] = LV_A$
        \item $\texttt{B} \in (CV_1.columns \cap CV_2.columns) $\\ $\Rightarrow CV_3[\texttt{B}] = CV_1[\texttt{B}] + CV_2[\texttt{B}] = LV_{B_1} + LV_{B_2}$
        \item $\texttt{C} \notin CV_1.columns \wedge \texttt{C} \in CV_2.columns $\\ $\Rightarrow CV_3[\texttt{C}] = CV_2[\texttt{C}] = LV_C$
        \item $CV_3 = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_{B_1} + LV_{B_2},\: \texttt{C}\!: LV_C\}$
    \end{enumerate}
\end{example-withrun}
% multiplication
\begin{example-withrun}
    Let us follow the construction of $CV_3$, that represents the column lineage embeddings of $t_1 \cdot t_2$ using Algorithm \ref{algo:mul_col_approx} (corresponds to joint use of data, i.e., AND in the query):
    \begin{enumerate}
        \item $CV_3 = \{\} \rightarrow \{\}$
        \item $CV_1.columns \,\cup\, CV_2.columns = \{\texttt{A}, \texttt{B}\} \cup \{\texttt{B}, \texttt{C}\} = \{\texttt{A}, \texttt{B}, \texttt{C}\}$
        \item $\texttt{A} \in CV_1.columns \wedge \texttt{A} \notin CV_2.columns $\\ $\Rightarrow CV_3[\texttt{A}] = CV_1[\texttt{A}] = LV_A$
        \item $\texttt{B} \in (CV_1.columns \cap CV_2.columns) $\\ $\Rightarrow CV_3[\texttt{B}] = CV_1[\texttt{B}] \cdot CV_2[\texttt{B}] = LV_{B_1} \cdot LV_{B_2}$
        \item $\texttt{C} \notin CV_1.columns \wedge \texttt{C} \in CV_2.columns $\\ $\Rightarrow CV_3[\texttt{C}] = CV_2[\texttt{C}] = LV_C$
        \item $CV_3 = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_{B_1} \cdot LV_{B_2},\: \texttt{C}\!: LV_C\}$
    \end{enumerate}
\end{example-withrun}


\subsubsection{Dropping lineage columns}\label{sec:cv_discussion}
% \begin{itemize}
$t.lineage\_columns$ (for a tuple $t$) might get large and include (almost) all the columns in the DB. This can render this solution impractical, since large modern systems may operate with hundreds and even more columns across the DB. There are various practical techniques that can serve to limit the number of lineage columns per tuple:
\begin{enumerate*}
    \item Set a bound \textit{b} on the number of $lineage\_columns$ (a hyperparameter).
    \item Give \textit{native priority}. That is, prefer keeping $native\_columns$ and cutting-off $inherited\_columns$, whose influence on \textit{this} tuple is more remote, when the bound is reached (see example \ref{example:generational_priority} below).
    \item Remove the relation name prefix from a column name, i.e., consider all $T.\texttt{Attr}$ as simply \texttt{Attr}. This might result in a loss of information, but hopefully not too harmful to the overall performance of the method.
\end{enumerate*}
Observe that the assumption in \ref{subsubsec:lineage-columns-filtering} of section \ref{sec:cv-implementation} breaks down under this lineage column cut-off technique. We can either live with the false negatives or suggest filtering only if the containment rate of $t'.lineage\_columns$ in $t.lineage\_columns$ is below some threshold.


% generational priority
\begin{example-withrun}\label{example:generational_priority}
    Let us follow the construction of $CV_3$, that represents the column lineage embeddings of $t_3 = t_1 + t_2$, such that the result is a new tuple $t_3 \in T_{AB}$ (a table with only two columns - \texttt{A} and \texttt{B}). In addition, we use a bound of $b = 2$ on the number of retained $lineage\_columns$ and implement native priority:
    \begin{enumerate}
        \item (see exapmle \ref{example:algo_add_col})\\ $CV_3 = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_{B_1} + LV_{B_2},\: \texttt{C}\!: LV_C\}$\\ $\Rightarrow t_3.lineage\_columns = \{\texttt{A}, \texttt{B}, \texttt{C}\}$
        \item $t_3 \in T_{AB}$ $\Rightarrow t_3.native\_columns = \{\texttt{A}, \texttt{B}\}$, \\$t_3.inherited\_columns = \{\texttt{C}\}$
        \item $|t_3.lineage\_columns| = 3 > 2 = b$
        \item $CV_3 = \{\texttt{A}\!: LV_A,\: \texttt{B}\!: LV_{B_1} + LV_{B_2}$\}\\ (the \textit{inherited\_column} \texttt{C} was eliminated)
    \end{enumerate}
\end{example-withrun}


% \subsection{Discussion} 
% % \begin{itemize}
% The rationale behind this method is partially inspired by the construction of ``tuple vectors'' by means of averaging the ``sentence vectors'' of the columns (as discussed in section \ref{sec:sentence_embeddings}).
% $t.lineage\_columns$ (for a tuple $t$) might get large and include (almost) all the columns in the DB. This can render this solution impractical, since large modern systems may operate with hundreds and even more columns across the DB. There are various practical techniques that can serve to limit the number of lineage columns per tuple:
% \begin{enumerate*}
%     \item Set a bound on the number of $lineage\_columns$ (a hyperparameter).
%     \item Give \textit{native priority}. That is, prefer keeping $native\_columns$ and cutting-off $inherited\_columns$, whose influence on \textit{this} tuple is more remote, when the bound is reached (see example \ref{example:generational_priority} above).
%     \item Remove the relation name prefix from a column name, i.e., consider all $T.\texttt{Attr}$ as simply \texttt{Attr}. This might result in a loss of information, but hopefully not too harmful to the overall performance of the method.
% \end{enumerate*}

% \subsection{Verifying the Lineage}
% Given a method that approximates the top-$n$ justifications for the existence of a query result tuple, as the one presented above, there is a simple technique to partially verify the collection of lineage candidates. The idea is applying the query $q$ that generated the tuple to be explained, $t$, to the collection of lineage tuples obtained by our system. If $t$ is output in the result of applying $q$ on these lineage candidates, then we found a sufficiently small (though, non-precise) explanation for $t$. Furthermore, one could utilize an exact provenance tracking application, e.g., ProvSQL \cite{provsql_github} by applying $q$ to the collection of tuples obtained by our technique, to explain $t$ (given that $t$ is ``verified''). This technique relies on the fact that executing $q$ on a small collection of tuples (even with exact provenance tracking) is significantly cheaper than applying the query on the whole, potentially large, DB.
    
% \end{itemize}


==> main/chap5_improving_lineage_embeddings.tex <==
\section{Improving Lineage Embeddings}
\label{chap:improving_lineage_embeddings}


\subsection{Tuple Creation Timestamp}
Filtering out non-lineage tuples by a tuple's creation timestamp is a good practice, and can help with filtering out very similar but non-lineage tuples, which might not be detected by the other methods. It is especially important for querying distant lineage (when the DB has existed for a sufficiently long time, so that a tuple's creation timestamp becomes a strong distinguishing factor).
% \\

% \subsubsection{Implementation} 
% \begin{enumerate}
%     \item Keep track of a tuple's creation timestamp:
%     \begin{itemize}
%         \item If a tuple $t$ was inserted explicitly to the DB then $t.timestamp$ is its insertion time.
%         \item If $t$ was calculated by a query, then $t.timestamp$ is the the query's execution time.
%     \end{itemize}
%     \item When comparing a tuple $t$ (and its lineage embeddings) to a set of other tuples $T'$, we can precede similarity calculations with the following step:
%     \begin{enumerate}
%         \item If $t'.timestamp > t.timestamp$ ($t' \in T'$) then $t'$ is newer than $t$ and therefore cannot be a part of its lineage.
%     \end{enumerate}
% \end{enumerate}


\subsection{Query-Dependent Column Weighting}\label{sec:query-dependent-weighting}
\subsubsection{Rationale} When analyzing lineage embeddings of query-result tuples against other tuples in the DB, we would like to emphasize certain \textit{columns of interest}. These columns can be derived from the structure of the query. For example, if a query asks for distinct manufacturer names of products that contain soda, then intuitively, we want the \texttt{manufacturer} and \texttt{ingredients} columns (of the \texttt{products} table) to have more influence on the respective lineage embeddings than other columns that are not mentioned in the query.

\subsubsection{Implementation} 
\begin{enumerate}
    \item Given a query $q$, we parse $q$ to retrieve the columns of interest and save them as additional meta information for every tuple in the result of $q$.
    \item When comparing a tuple from the result of $q$ with another tuple from the DB, we compare between respective column vectors and calculate a weighted average of the similarities while prioritizing the columns of interest. For example, say a tuple $t$ that has lineage vectors for columns \texttt{A},\texttt{B} was created by a query $q$, such that $q.cols\_of\_interest$ = \{\texttt{B}\}; and we compare $t$ with another tuple $t'$ that has lineage vectors for columns \texttt{A},\texttt{B}:
    \begin{equation*}
        \operatorname{sim}(t, t') = \frac{w_\texttt{A}*\operatorname{sim}(t.\texttt{A}, t'.\texttt{A}) +
        w_\texttt{B}*\operatorname{sim}(t.\texttt{B}, t'.\texttt{B})}{w_\texttt{A} + w_\texttt{B}}
    \end{equation*}
    where $w_\texttt{A}$ and $w_\texttt{B}$ are respective column weights such that $w_\texttt{B} > w_\texttt{A}$ as column \texttt{B} is mentioned in the query. $\operatorname{sim}(t.\texttt{A}, t'.\texttt{A})$ is the calculated similarity between the lineage vectors for column \texttt{A} of $t$ and $t'$ (similarly for column \texttt{B}). Observe that although column \texttt{A} is not a column of interest in the example, it is a mutual ``gene'' of tuples $t$ and $t'$, and, thus it still holds lineage information that is valuable to the similarity calculation.
\end{enumerate}

\subsubsection{Note} This technique is applicable mainly for \textit{direct} lineage. In the context of distant lineage we can use it to get ``immediate contributors'' but also take into account lineage tuples identified without this technique (they will naturally tend to be ranked lower).
 


% \subsection{Bloom-Filters of Queries}\label{sec:bloom-filters}
% \subsubsection{Rationale} We would like to distinguish between very similar/nearly identical tuples (text-wise). The main idea here is keeping additional information per-tuple, that encodes the queries that had the tuple in their lineage (i.e., for every tuple $t$ - keep track of every query $q$, such that $t$ was involved meaningfully in the evaluation of $q$). Also, for each query-inserted tuple $t$ record the query $q$ that inserted it. This approach enables us to filter out (in a probabilistic manner) tuples that were not involved meaningfully in the evaluation of a query, since Bloom Filters do not produce false negatives (in our case, a false negative is a tuple $t$ that \textbf{was} involved in the evaluation of a query $q$, but $q \notin t.bloom\_filter$).

% \subsubsection{Implementation}  
% \begin{enumerate}
%     \item Initialize a Scalable Bloom Filter \cite{scalable-bloom-filters} of size $B$ (a hyperparameter) for every tuple in the DB.
%     \item For every tuple $t$ that is involved meaningfully in the evaluation of a query $q$: insert $q$ (hashed) to $t$'s Bloom filter.
%     \item When comparing a tuple $t$ (and its lineage embeddings) that was created by a query $q$ (as recorded with this tuple) to a set of other tuples $T'$, we can precede similarity calculations with the following step:
%     if $q \notin t'.bloom\_filter$ then $t'$ was definitely not involved in the evaluation of $q$. Thus, it cannot be a part of $t$'s \textbf{direct} lineage.
%     \item Several optimizations and design choices were made to enforce a size-bounded lineage representation while using Scalable Bloom filters, as detailed in the preliminary work \cite{DBLP:conf/vldb/LeybovichS20}.
    
    % Therefore, it seems that using a Scalable Bloom filter (per-tuple) contradicts this notion, as its size is ultimately bounded by the number of queries served by the system. Therefore, we devise a ``switch \& reset policy'' for these bloom filters:
    % \begin{enumerate*}
    %     \item Instead of only one Bloom filter - maintain two Bloom filters per-tuple (we fill them both).
    %     \item One filter is ``big and old'' and one is ``small and young''.
    %     \item Lineage ``filtering'' is done against the old one.
    %     \item Once the young one has seen sufficiently many queries - we switch to the young one and recycle the old filter. We then call the young old and create a new (empty) young filter.
    %     \item This way we lose information but only about relatively ``old'' queries.
    %     \item In order to maintain the invariant of ``no false negatives'' when querying the old Bloom filter of a tuple $t$ - it is important to keep track of the oldest query id that is tracked by the old filter. That is, say the current old filter of $t$ encodes information only for queries $q$ with $q.id \geq t.oldest\_query\_id$ (we view query id's as timestamps); then given a tuple $t'$ which was created by a query $q'$ with $q'.id < t.oldest\_query\_id$ - we do not test for the existence of $q'$ in $t.bloom\_filter$ (otherwise, we risk returning a false negative).
        
    %     % \footnotetext{We view query id's as timestamps.}
    % \end{enumerate*}
    % \begin{enumerate}
    %     \item If $q \notin t'.bloom\_filter$ then $t'$ was definitely not involved in the evaluation of $q$. Thus, it cannot be a part of $t$'s \textbf{direct} lineage.
    % \end{enumerate}
% \end{enumerate}

% \subsubsection{Distant lineage perspective}
% This technique filters tuples that were not \textit{directly} involved in the evaluation of a query; hence, it is not applicable to distant (indirect) lineage. A possible direction of extending the basic method is a recursive algorithm that takes into account the query that produced each already discovered (presumed lineage) tuple.

% \subsubsection{Note} 
% % \begin{enumerate*}
%     % \item This technique filters tuples that were not \textit{directly} involved in the evaluation of a query; hence, it is not applicable to distant (indirect) lineage. A possible direction of extending the basic method is a recursive algorithm that takes into account the query that produced each already discovered (presumed lineage) tuple.
%     % \item Bloom Filters are probabilistic, but they do not produce false negatives. Thus, they can be reliably used to filter out non-lineage tuples (in our case, a false negative is a tuple $t$ that \textbf{was} involved in the evaluation of a query $q$, but $q \notin t.bloom\_filter$). 
%     % \item We emphasize a size-bounded lineage representation. Therefore, it seems that using a Scalable Bloom filter (per-tuple) contradicts this notion, as its size is ultimately bounded by the number of queries served by the system. Therefore, we devise a ``switch \& reset policy'' for these bloom filters:
%     % \begin{enumerate*}
%     %     \item Instead of only one Bloom filter - maintain two Bloom filters per-tuple (we fill them both).
%     %     \item One filter is ``big and old'' and one is ``small and young''.
%     %     \item Lineage ``filtering'' is done against the old one.
%     %     \item Once the young one has seen sufficiently many queries - we switch to the young one and recycle the old filter. We then call the young old and create a new (empty) young filter.
%     %     \item This way we lose information but only about relatively ``old'' queries.
%     %     \item In order to maintain the invariant of ``no false negatives'' when querying the old Bloom filter of a tuple $t$ - it is important to keep track of the oldest query id that is tracked by the old filter. That is, say the current old filter of $t$ encodes information only for queries $q$ with $q.id \geq t.oldest\_query\_id$\footnotemark; then given a tuple $t'$ which was created by a query $q'$ with $q'.id < t.oldest\_query\_id$ - we do not test for the existence of $q'$ in $t.bloom\_filter$ (otherwise, we risk returning a false negative).
%     %     \footnotetext{We view query id's as timestamps.}
%     % \end{enumerate*}
%     Bloom Filters are a universal enhancement that can be applied to any lineage-approximation technique. They complement beautifully the word embedding based lineage vectors, but are far from being a ``silver bullet'' on their own. In particular, in the extreme case where most (or even all) the tuples of a table \texttt{A} participate in the evaluation of a query $q$, the Bloom Filters (almost) will not help when comparing a tuple from the result of $q$ to tuples from table \texttt{A}.
% % \end{enumerate*}


\subsection{Weighting with Query Dependency DAG}
\subsubsection{Rationale} We would like to distinguish between very similar/nearly identical tuples (text-wise) during both direct and distant lineage querying. 
Additionally, we want to enhance the natural ranking of lineage tuples by amplifying the ``generational gaps''. The idea is that tuples from earlier generations in the distant lineage tree structure (of a query-inserted tuple) are to be assigned a lower similarity score during distant lineage querying. 
The technique is keeping track of \textit{dependencies between queries} in a DAG structure and weighting the similarity scores of query-inserted tuples (during lineage querying) inversely proportional to the distance, between their inserting queries to the query that computed the explained tuple, in the query dependency DAG. We say that a query $q$ \textit{depends on} a query $p$ if a tuple $t_p$ that was created by $p$ was meaningfully involved in the evaluation of $q$ (i.e., $t_p$ is in the distant lineage of some result tuple $t_q$ in the result of $q$).
This approach enables us to give lower similarity scores to tuples that were not involved meaningfully in the evaluation of a query (directly or remotely) and amplify the natural ranking of the results in terms of query creation dependencies.

\subsubsection{Implementation}
\begin{enumerate}
    \item If there is a tuple $t_p$ that is involved meaningfully in the evaluation of a query $q$: we say that $q$ \textit{depends on} the query $p$ that inserted $t_p$ into the DB.
    \item Initialize an empty query dependency DAG $G = (V, E)$ with a maximum number of nodes $S$ and a maximum height $H$ (hyperparameters), such that $V$ is a set of queries and $E = \{(q, p) \in V\! \times\!V\; |\; q\: depends\: on\: p\}$. 
    % \item Maintain a hash table of queries, for a quick look-up of nodes in the query dependency graph.
    % \item Maintain a linked list of queries that is sorted by query execution order (oldest to newest). This list helps us to quickly find the ``oldest'' queries that need to be removed from the graph, when the size limit $S$ is reached.
    \item When comparing a tuple $t_q$ (and its lineage embeddings) that was created by a query $q$ (as recorded with this tuple) to another tuple $t_p$ in the DB, we can \textbf{replace} similarity calculations with the following steps:
    \begin{enumerate}
        \item Denote the sub-tree of $q$ in $G$ (i.e., rooted at $q$) as $G_q = (V_q, E_q)$.
        \item Denote the query that created the tuple $t_p$ (as recorded with this tuple) as $p$.
        \item If $p \in V_q$ then multiply the similarity for $t_p$ by $w_d \leq 1$, which is inversely proportional to the distance $d$ from $q$ to $p$ in $G_q$. One possible implementation for the distance-dependent weighting is $w_d = max\{\frac{1}{2}, 1 - \frac{(d - 1)}{10}\}$, such that $w_1 = 1$, $w_2 = \frac{9}{10}$, etc., and $\forall 1\leq d\leq H: w_d \geq \frac{1}{2}$. Other implementations exist as well. 
        \item If $p \notin V_q$ then multiply the similarity for $t_p$ by $0 <$ $w_{outsider} <$ $w_{d=H}$ (a hyperparameter). Note that since we defined limits on the maximum number of nodes $S$ and maximum height $H$, some nodes will need to be removed when those limits are reached (see details below). Thus, this method might start producing false negatives at some point; and to not lose those tuples completely, we choose to multiply their similarity by some small, non-zero constant, instead of plainly filtering them out.
    \end{enumerate}
    \item We emphasize a lineage tracking system with constant additional space per tuple. The query dependency DAG adheres to this philosophy and is limited in size by the hyperparameters $S$ and $H$. Several design choices were made to enforce these limits, while maintaining effectiveness.
\end{enumerate}

% \subsubsection{Additional Design Choices} 
% \begin{itemize}
%     \item With each node in the graph $G$ we keep additional information about its height. This information is maintained and updated upon new edge additions to $G$.
%     \item Maintain a hash table of queries, for a quick look-up of nodes in the query dependency graph.
%     \item Maintain a doubly linked list of queries that is sorted by query execution order (oldest to newest). This list helps us to quickly find the ``oldest'' queries that need to be removed from the graph, when the cardinality limit $S$ is reached.
%     \item When the height limit $H$ is reached, we eliminate ``deep'' leaves (those are the oldest queries in a given branch).
%     \item In this work we emphasize a lineage tracking system with constant additional space per tuple. The query dependency DAG adheres to the same philosophy and is limited in size by the hyperparameters $S$ and $H$.
% \end{itemize}


% \subsection{Limit Provenance Analysis to Specific Base Tables}

% \subsubsection{Rationale}
% % use case for an analyst
% We consider those tables that do not depend on the contents of the DB when these tables are created, and thereafter, as \textit{base tables}. Note that tuples can be manually inserted to and deleted from base tables, but, not in a programmatic manner over the DB, e.g., a SQL \texttt{INSERT} statement that is based on the DB contents.
% At times, an analyst might be interested only in a \textbf{subset of base tables} for lineage analysis of tuples that were created by a query. That is, an analyst's workflow may be comprised of the following steps:
% \begin{enumerate}
%     \item Choose a tuple of interest $t$ that was created by a query - for analysis.
%     \item Compare the tuple $t$ (via lineage vectors) to tuples from a pre-defined subset of the base tables (e.g., $\{{A, B}\} \subset \{{A,B,C,D,E}\}$, where $A,B,C,D,E$ are base relations in the DB).
%     \item Find the Top-$K$ ($K$ is a parameter) source tuples (by similarity) that were meaningfully involved in the creation of $t$. 
% \end{enumerate}

% This workflow seems useful and worthy of consideration. Note that it entails a relaxed assumption about the lineage analysis requirements in our system, and we would like to exploit it to produce better (i.e., more precise) answers.
% % how it (should) helps precision
% \par A modern DB may include a large number of base tables, and new tuples that are created from base tables (by a query). As time goes on and the queries become more complex and involve (directly or indirectly) more base tables - we anticipate a growing amount of ``noise'' in the lineage vectors that we maintain.
% Given an assumption that an analyst is only interested in a (relatively small) subset of the base tables for lineage analysis, we hypothesize that it is possible to diminish the amount of ``noise'' that we propagate over time (via the lineage vectors) by limiting lineage tracking to tuples from base tables that are of interest to the analyst, and tuples that are created from them (by queries).

% \subsubsection{Implementation}
% This technique can be implemented as a wrapper to the addition and multiplication operations on lineage vectors, as presented previously in Algorithms \ref{algo:add_approx} and \ref{algo:mul_approx}: 
% \begin{enumerate}
%     \item Denote the subset of base tables that is of interest to the analyst as $S$.
%     \item For each tuple $t$, define $t.related\_tables = \{T'\; |\; \exists t' \in T': t'$ is in the distant lineage of $t\}$. That is, all the tables that were involved (directly or indirectly) in the evaluation of $t$.
%     \item Suppose we are given two tuples $t_1$ and $t_2$ with corresponding sets of lineage vectors $LV_1$ and $LV_2$ (either tuple vectors, or column vectors for a specific column) and an operation $op \in \{+, \cdot\}$, such that we are interested in calculating $LV_1 \; op \; LV_2$.
%     \item If $t_1.related\_tables \cap S \neq \emptyset$ and $t_2.related\_tables \cap S \neq \emptyset$, then we proceed as usual, namely, return $LV_1 \; op \; LV_2$. 
%     \item Otherwise, if only one of $t_1, t_2$ has related tables in $S$, i.e., suppose without loss of generality that $t_1.related\_tables \cap S \neq \emptyset$ and $t_2.related\_tables \cap S = \emptyset$ then we return $LV_1$.
%     That is, we propagate forward only the relevant lineage data.
%     \item Otherwise, if both $t1$ and $t2$ are of no interest to an analyst, then the output value is of no relevance either, and no vector calculation is performed.
% \end{enumerate}

% \subsubsection{Notes}
% \begin{itemize}
%     \item Borrowing from semiring theory, this technique is analogous to tagging each ``irrelevant'' base tuple as additive and multiplicative identity in terms of lineage vectors operations.
%     \item Propagating the ``related tables'' information (during lineage vectors computation) is essential for the correctness of this method.
%     \item Suppose there are analysts $A_1, ..., A_m$ each with their own set of base tables of interest $B_1, ..., B_m$.
%     Then, we may conceivably apply this technique separately to each $A_i$ and $B_i$ (of course, with the implied storage overhead).
% \end{itemize}


% \subsection{Where Provenance}
% Recording lineage vectors per fully named columns (see chapter \ref{chap:per_column_lineage_vectors}) enables implementing a form of \textit{where provenance} (we are only interested in non-distant provenance here). By where provenance we mean the following. Given a tuple $t$ in relation $T$ of the DB, a native column \texttt{A} in $t$ and a value $v_\texttt{A}$ for $t$ in column $T.\texttt{A}$, determine the likely tuples $t’$, the \textit{where tuples} in the DB, from which the value $v_\texttt{A}$ originated. If the \texttt{SELECT} clause of $q$, the query that inserted $t$ into the DB, indicates an assigned constant, then no such where tuples exist. 
% \par Otherwise, the technique for locating likely where tuples explaining $v_\texttt{A}$ is as follows. Let $CV_t$ be the mapping associated with the tuple $t$:
% \begin{enumerate}
%     \item Find the where tuples \textit{candidates} by analyzing the structure of $q$, the query that inserted $t$ into the DB. That is, if $q$ indicates in the \texttt{SELECT} clause that $T'.\texttt{A}'$ is assigned to $T.\texttt{A}$, then the candidates are the tuples $t' \in T'$ that agree with $t$ on the value of $v_\texttt{A}$ (i.e., $v'_{\texttt{A}'}$ = $v_\texttt{A}$, where $v'_{\texttt{A}'}$ is the value for $t'$ in column $T'.\texttt{A}'$). 
%     Note that: 
%     \begin{itemize}
%         \item If the \texttt{SELECT} clause of $q$ contains other columns from $T'$, e.g., the column $T'.\texttt{B}'$ is assigned to $T.\texttt{B}$, then additional filtering of candidate where tuples is possible, as these tuples must agree with $t$ on the respective value $v_\texttt{B}$ of tuple $t$ for column $T.\texttt{B}$ as well. 
%         \item If $q$ indicates in the \texttt{SELECT} clause that $T.\texttt{A}$ is assigned to by combining multiple columns, e.g., $T'_1.\texttt{A}'_1$ $*$ $T'_2.\texttt{A}'_2$ is assigned to $T.\texttt{A}$, then the candidates are the tuples $t'_1 \in T'_1$ and $t'_2 \in T'_2$ that (when combined) agree with $t$ on the value of $v_\texttt{A}$ (i.e., $v'_{\texttt{A}'_1} * v'_{\texttt{A}'_2}$ = $v_\texttt{A}$, where $v'_{\texttt{A}'_i}$ is the value for $t'_i$ in column $T'_i.\texttt{A}'_i$). 
%     \end{itemize}
%     \item A where tuple needs be directly involved in the computation of $t$, namely used by the query $q$ that inserted $t$ into the DB.
%     This information is encoded both in $t'$'s Bloom Filter of queries and the query dependency DAG (some redundancy, though the Bloom Filter is more precise in this regard).
%     So, if $q \notin t'.bloom\_filter$ or if $t’$ was inserted by a query $p$ and $(q,p)$ is not an edge in the query dependency DAG, $t’$ cannot be a where tuple explaining $v_\texttt{A}$ in $T.\texttt{A}$.
%     \item To test closeness between $t$ and a candidate where tuple $t'$, we simply calculate $\operatorname{sim}$($t$, $t’$), the similarity between these two tuples, using the mappings $CV_t$ and $CV_{t'}$ associated with $t$ and $t'$, respectively (as explained in chapter \ref{chap:per_column_lineage_vectors}). Intuitively, it is more beneficial to consider the full mappings $CV_t$ and $CV_{t'}$, when testing closeness between $t$ and $t'$, instead of just comparing $CV_t[T.A]$ and $CV_{t'}[T'.A']$. The reason is that the full mappings usually contain additional useful information, based on which the candidates can be compared and better differentiated.
% \end{enumerate}


==> main/chap6_experimental_evaluation.tex <==
\section{Experimental Evaluation}
\label{chap:experimental_evaluation}

In this section we first establish an explanation quality measure, in terms of precision and per-level recall. We then present and analyze results of our approximate lineage system experimentation against an ``exact provenance tracking system'' - ProvSQL.


\subsection{Experimental Setup}\label{sec:evaluation-setup}
% We used two datasets from different domains (food and movies) to compare the performance of our approximate lineage system against ProvSQL. The goal of these experiments is evaluating the precision of our approximate explanations against an ``exact provenance tracking system''.
\par\textbf{Note.} \textit{max\_vectors\_num} (see section \ref{sec:proposed_solution_approx}) was chosen manually to be 4. The choice of hyperparameters, and, specifically, \textit{max\_vectors\_num} - is the subject of ongoing research.\\

% USDA BFPD and MovieLens
% \subsubsection{Datasets}\label{sec:datasets}
% \begin{enumerate}
%     \item The USDA Branded Food Products Database (BFPDB) \cite{usda_bfpd-dataset} is the result of a Public-Private Partnership, whose goal is to enhance public health and the sharing of open data by complementing USDA Food Composition Databases with nutrient composition of branded foods and private label data, provided by the food industry. Among others, the dataset includes three tables:
%     \begin{itemize}
%         \item \texttt{products} - contains basic information on branded products (manufacturer, name, ingredients).
%         \item \texttt{nutrients} - each tuple contains all nutrient value information about a product.
%         \item \texttt{serving\_size} - each tuple contains information about a product's serving size (as well as unit of measurement) and food preparation state.
%         \item \texttt{derivation\_code\_description} - contains all nutrient derivation codes and their detailed descriptions.
%     \end{itemize}
%     Each product in the BFPDB dataset has a unique identifier, \texttt{ndb\_no}. 
%     % For a detailed description of the BFPDB dataset see appendix \ref{appendix:bfpdb_schema}.
    
%     \item The MovieLens dataset \cite{movielens-dataset} describes people’s preferences for movies. These preferences are entered by way of the MovieLens website \cite{movielens-recommender-website} — a recommender system that asks its users to provide movie ratings in order to receive personalized movie recommendations. Among others, the dataset includes three tables:
%     \begin{itemize}
%         \item \texttt{movies} - each tuple contains basic information about a movie (title, genres).
%         \item \texttt{ratings} - each tuple contains information about a user's expressed preference of a movie (a 0-5 star rating).
%         \item \texttt{tags} - each tuple contains information about a user's classification tag of a movie (silly, funny, etc.).
%     \end{itemize}
%     Each movie in the MovieLens dataset has a unique identifier, \texttt{movieId}. 
%     % For a detailed description of the MovieLens dataset see appendix \ref{appendix:movielens_schema}.
% \end{enumerate}

% Explain how the precision evaluation process works (test against lineage from provsql)
\subsubsection{Precision Calculation}\label{sec:precision}
As stated in section \ref{sec:proposed_solution_approx}, we expect our explanations to approximate the exact lineage of query result tuples. 
Thus, in order to test the aforementioned algorithms and implementation, we devised an explanation quality measure for explaining a single tuple $t$, where $k$ is a parameter: 
\begin{equation*}
    \operatorname{Precision}(t, k) = \frac{|ApproxLineage(t, k) \cap ExactLineage(t)|}{|ApproxLineage(t, k)|}
\end{equation*}
where $ApproxLineage(t, k)$ is the set of the top $k$ (by lineage similarity) tuples, returned as explanations (i.e., approximate lineage) for $t$ by our system. $ExactLineage(t)$ is the set of tuples that comprise the exact \textbf{distant} lineage of $t$, it can be calculated recursively from the semiring polynomial that is returned by the ProvSQL system for $t$.
For example, if the direct lineage of $t_4$ and $t_5$ are the sets $\{t_1, t_2, t_3\}$ and $\{t_1\}$, respectively, and the direct lineage of a tuple $t_6$ is the set $\{t_4, t_5\}$ then the total distant lineage for the tuple $t_6$ is $\{t_1, t_2, t_3, t_4, t_5\}$.
The parameter $k$ is set by us in each experiment, that is, it is a parameter of the experiment. 
$\operatorname{Precision(t, k)}$ is tunable via the parameter $k$, i.e., when $k$ is small we test for precision of the ``top'' explanations we found.
\par Classically, we are usually interested in precision and recall (e.g., in traditional statistics and classification problems). However, here the situation is slightly different, what we really are interested in is to assess the quality of our explanations by measuring ``how many of the top $k$ (by lineage similarity) tuples are actually part of the exact lineage?''. By contrast, traditional recall does not seem to be a meaningful metric in our case, as many query-result tuples might have long histories. Hence, a top-$k$ justifications result is preferred over ``returning all the correct lineage tuples'', and this is what we measure.

\subsubsection{Distant Lineage: Per-Level Recall}\label{sec:recall}
    In order to assess the quality of a distant lineage answer in a more insightful way, in the experiments we save the ``exact distant lineage'' in a hierarchical structure, and analyze it per-level. Consider a list $L$ of sets per-tuple, s.t. $L[i]$ is the set of all lineage tuples at the $i^{th}$ derivation depth level. Note that $i$ starts at $0$, s.t. the $0^{th}$ lineage level is a set containing the target tuple only. For example, if the direct lineage of $t_4$ and $t_5$ are the sets $\{t_1, t_2, t_3\}$ and $\{t_1\}$, respectively, and the direct lineage of a tuple $t_6$ is the set $\{t_3, t_4, t_5\}$ (note that $t_3$ appears in both the $1^{st}$ and the $2^{nd}$ lineage levels of $t_6$, in this example) then the hierarchical lineage DAG for the tuple $t_6$, and the hierarchical list structure that represents it, look as follows: \\\\
    \input{figures/distant_lineage_tree} \hspace{35pt}
    \input{figures/distant_lineage_list} \\\\
Here, each rectangle is an entry in the list $L$.
\par We expect our explanations to have a ``natural ranking'' property in terms of lineage levels. That is, we expect the similarity between a target tuple and tuples in its distant lineage to be inversely related to the distance between them in the hierarchical lineage DAG structure. Thus, we devise an explanation quality measure $\operatorname{Recall}(t, i)$ for the explanation of a single tuple $t$ and its lineage level $i$. Let $D(t, i)$ be the number of unique returned tuples in the exact lineage of $t$ up until the $i^{th}$ level (including); formally, $D(t, i) = |\bigcup\limits_{j=1}^{i} L_t[j]|$. Define
\begin{equation*}
    \operatorname{Recall}(t, i) = \frac{|ApproxLineage(t, D(t, i)) \cap L_t[i])|}{|L_t[i]|}
\end{equation*}
where $ApproxLineage(t, D(t, i))$ is the set of the top $D(t, i)$ (by lineage similarity) tuples, returned as explanations (i.e., approximate lineage) for $t$ by our system.
% $D(t, i)$ is the number of unique returned tuples in the exact lineage of $t$ up until the $i^{th}$ level (including). Formally, it is defined as follows: $D(t, i) = |\bigcup\limits_{j=1}^{i} L_t[j]|$.
$L_t$ is the hierarchical list structure for $t$, as defined above, i.e., $L_t[i]$ is the set of all lineage tuples at the $i^{th}$ derivation depth level of $t$.

% \subsection{Initial Experiments}\label{sec:initial-experimentation}
% In \cite{DBLP:conf/vldb/LeybovichS20} we present initial experimentation results on both the MovieLens \cite{movielens-dataset} and BFPDB \cite{usda_bfpd-dataset} datasets. These experiments focus on \textbf{direct} lineage analysis, comparing per-tuple lineage vectors with per-column lineage vectors, and exhibit the usefulness of improvements suggested in section \ref{chap:improving_lineage_embeddings}, such as Bloom-Filters of queries.

% Having established an explanation quality measure, we conducted a series of experiments. In particular, we tested the precision of direct provenance of different queries, varying from ``simple'' (examples \ref{experiment:1} and \ref{experiment:2}) to ``complex'' (example \ref{experiment:3}) queries. We show some of the experimental results and present a qualitative analysis.
% \par\textbf{Note.} In all the examples, the lineage (and its size - `Lin. size' column) of a tuple, is calculated as a subset of the exact lineage. That is, if we compare a query result tuple with $\texttt{products}.tuples$, i.e., all the tuples in the \texttt{products} table (in order to find the top $k$ most similar tuples) - we use only \texttt{product} tuples in the exact lineage for precision calculations ($Lineage\_products(t)$ = $ExactLineage(t) \cap \texttt{products}.tuples$).


% \begin{runexample}
% We test queries on a small subset of the MovieLens dataset. Each table (i.e., \texttt{movies}, \texttt{ratings}, \texttt{tags}) consists of about 10,000 tuples.
% \end{runexample}
% %%% Present here all the queries? Figure? I think NO

% % Example 1
% % MovieLens tuples vs. columns.
% % \input{tables/example1}
% % ''Toy'' example
% \begin{example-withrun}\label{experiment:1}
% \input{tables/example1}
% \footnotetext{$Lineage\_tags(t) = ExactLineage(t) \cap \texttt{tags}.tuples$.}
% \input{tables/example2}
% \input{tables/example3}
% We ask for distinct \texttt{users} that tagged a Comedy/Romance genre \texttt{movie} as one of \textit{funny}, \textit{superhero}, \textit{family}, \textit{music}. The results are shown in Table \ref{tab:1}. Precision calculation is discussed in section \ref{sec:evaluation-setup}. The approximate lineage is calculated from comparing result tuples to tuples from the \texttt{tags} table (see preceding Note). Right away, it is evident that provenance column vectors produce better approximate lineages than tuple vectors.\\
% \par In this example tuples No.\texttt{0} and No.\texttt{6} display superior precision for column vectors. Tuple No.\texttt{7} is  interesting as it is a case of lineage size $>$ 1 for which both methods (tuple and column vectors) produce an accuracy of 1.0.
% It is interesting to examine tuple No.\texttt{7} more closely to gain a better grasp of the differences between tuple and column vectors.
% Now, let us analyze the top \textbf{3} (by similarity) tuples from the \texttt{tags} table, which are returned by our system for tuple No.\texttt{7} in Table \ref{tab:1} (\texttt{userId}=282405, Lin. size=\textbf{2}) for both the tuple-based and column vectors-based methods:\\\\\\
% \par\textbf{Tuple Vectors:}\\
% \input{tables/res2}\\
% \par\textbf{Column Vectors:}\\
% \input{tables/res1}
% \\
% As shown in the two tables above, both methods give maximal similarity (top 2) for the correct tuples in the exact lineage. However, the ``column vectors'' method produces better separation ($0.94-0.89 = 0.05$ vs. $0.88-0.86=0.02$) in terms of similarity between correct and incorrect lineage tuples. Another interesting point of distinction between the two methods is the 3$^{rd}$ most similar tuple returned:
% \begin{itemize}
%     \item The ``tuple vectors'' method returns a tuple which describes a tag of a correct movie (Zootopia) by the correct user (282405) with an incorrect label - \textit{acceptance}.
%     \item The ``column vectors'' method returns a tuple which describes a tag of an incorrect movie (Coco - not a Romance/Comedy movie) by the correct user (282405) with a correct label - \textit{music}.
% \end{itemize}
% The reason for this dissimilarity in behavior might be the result of giving the \texttt{tag} column more weight when comparing lineage column vectors (as discussed in section \ref{sec:query-dependent-weighting}).

% \end{example-withrun}


% \begin{runexample}
% We test queries on a small subset of the BFPDB dataset. Each table (\texttt{products}, \texttt{nutrients}, \texttt{serving\_size}) consists of about 10,000 tuples.
% \end{runexample}

% % Example 2
% % BFPD tuples vs. columns.
% % Examine top mistakes and discuss column weighting.
% \begin{example-withrun}\label{experiment:2}
% % \input{tables/example2}
% We ask for distinct \texttt{manufacturers} of products that have \textit{cholesterol} value information in the \texttt{nutrients} table. Let us first look at the query:
% \input{figures/q1}

% Now, by parsing the query we conclude that the columns \texttt{ndb\_no, nutrient\_name, manufacturer} are the ``columns of interest'' (discussed in section \ref{sec:query-dependent-weighting}). Thus, when comparing lineage column vectors of a query result tuple with another tuple from the DB - we give the columns of interest more weight. The results (and comparisons between the different techniques) are shown in Table \ref{tab:2}. The approximate lineage is calculated from comparing result tuples to tuples from the \texttt{nutrients} table. As evident from the presented results, incorporating query-based column weighting can significantly improve the precision of our system. 
% \par\textbf{Note.} This example displays lineage querying for result tuples with more than just a few tuples in their exact lineage (i.e., up to two hundreds).

% \end{example-withrun}

% % Example 3
% % BFPD tuples vs. columns vs. Bloom
% % Explain why Bloom helps
% \begin{example-withrun}\label{experiment:3}
% % \input{tables/example3}
% We ask for distinct \texttt{manufacturers} of products that have \textit{reeses} in their name and contain \textit{protein}
%                          \texttt{nutrient} information.
%                 Also, these \texttt{manufacturers} must produce \textit{unprepared} \texttt{products} (this information is stored in the \texttt{serving\_size} table).
% The only \texttt{manufacturer} in the BFPDB dataset that satisfies the (albeit a complex one) query is \textit{general mills sales}. Moreover, its exact lineage size (obtained by ProvSQL) is a relatively big number - \textbf{1966}; hence, it makes an interesting case study for the existence of drift errors in the construction of lineage vectors. That is, there is a potential for noise accumulation when combining a large number of lineage vectors with $+,\cdot$ and clustering operations (as discussed in section \ref{sec:proposed_solution_approx}). 
% The results are shown in Table \ref{tab:3}. The approximate lineage is calculated from comparing result tuples to tuples from the \texttt{serving\_size} table. As evident from the results, our solution (with query-based weighted column vectors and Bloom filters of queries) does not suffer from drift errors (limiting drift errors for distant provenance and direct provenance at scale are the subjects of ongoing research).
% \par\textbf{Notes.} 
% \begin{itemize}
%     \item The query-result tuple for \textit{general mills sales} has a lineage of size 1966, which is ${\sim}20\%$ of the tuples in the \texttt{serving\_size} table in our experiments (in a production setting, it can be orders of magnitude larger). Instead, we approximate the lineage with a small (and bounded) number of vectors. We argue that if lineage is huge our method makes more sense for direct provenance calculation than exact lineage calculations.
%     \item In this example the query accesses three tables in a non-trivial way, which suggests the way more complex queries would behave.
% \end{itemize}

% \footnotetext{
% $Lineage\_nutrients(t) = ExactLineage(t) \cap \texttt{nutrients}.tuples.$
% }
% \end{example-withrun}


\subsection{Experimenting with Direct and Multi-Generation Lineage}\label{sec:advanced_experiments}
% Explain what this section will contain - mainly, distant lineage testing
In this section we focus on tuples with multiple generations in their lifelong lineage history and analyze them in terms of direct and \textbf{distant} lineage.
We assess the performance of our system quantitatively using precision and per-level recall (see sections \ref{sec:precision} and \ref{sec:recall}, respectively) and qualitatively by observing the ``top-$k$'' returned lineage tuples (by similarity).
\par Note that
suggested improvements (section \ref{chap:improving_lineage_embeddings}) such as query-dependent column weighting, tuple creation timestamp and weighting with query dependency DAG are used (in the following experiments) for both the Tuple Vectors and the Column Vectors approximate lineage computation methods.

\subsubsection{The BFPDB Dataset}
The USDA Branded Food Products Database (BFPDB) \cite{usda_bfpd-dataset} is the result of a Public-Private Partnership, whose goal is to enhance public health and the sharing of open data by complementing USDA Food Composition Databases with nutrient composition of branded foods and private label data, provided by the food industry. Among others, the dataset includes three tables:
    \begin{enumerate*}
        \item \texttt{products} - contains basic information on branded products (manufacturer, name, ingredients).
        \item \texttt{nutrients} - each tuple contains all nutrient value information about some product.
        \item \texttt{serving\_size} - each tuple contains information about a product's serving size (as well as unit of measurement) and food preparation state.
        % \item \texttt{derivation\_code\_description} - contains all nutrient derivation codes and their detailed descriptions.
    \end{enumerate*}
    Each product in the BFPDB dataset has a unique identifier, \texttt{ndb\_no}.


\subsubsection{A Hierarchy of Materialized Views}
% Present and explain the hierarchy - like in github but more in detail.
We want to simulate a DBMS that contains a significant portion of tuples that depend on the contents of the DB, as a \textit{platform} for testing and analyzing distant lineage. Thus, we built a hierarchy of ``materialized views'', such that each ``view'' is a table, constructed from tuples that were generated by a single query.
In particular, we detail the following materialized views (the text colors are intended as a visual aid, such that each lineage generation has a brighter color, the farther it is from the base relations):
\begin{enumerate*}
    % \item \textcolor{Orchid}{\texttt{readytodrink}} was directly created from tuples of the tables \textcolor{Violet}{\texttt{products}} and \textcolor{Violet}{\texttt{serving\_size}}.
    % \item \texttt{prepared} and \texttt{unprepared} were directly created from tuples from the tables \texttt{products} and \texttt{serving\_size}.
    % \item \texttt{protein} was directly created from tuples from the tables \texttt{products} and \texttt{nutrients}.
    \item \textcolor{Orchid}{\texttt{sugars}} was directly created from tuples of the tables \textcolor{Violet}{\texttt{products}} and \textcolor{Violet}{\texttt{nutrients}}. It contains all the products-related information from the \texttt{products} table, for products that have a \textit{sugars} nutrient-related information in the \texttt{nutrients} table.
    % \item $\texttt{exp}\sb\texttt{1}$ was directly created from tuples from the materialized views \texttt{prepared} and \texttt{protein}. 
    \item \textcolor{CarnationPink}{$\texttt{exp}\sb\texttt{2}$} was directly created from tuples of the materialized views \textcolor{Orchid}{\texttt{unprepared}} and \textcolor{Orchid}{\texttt{protein}}. It contains distinct manufacturers of products that have \textit{water} as an ingredient, and contain \textit{protein} nutrient information; also, these manufacturers produce \textit{unprepared} products.
    \item \textcolor{CarnationPink}{$\texttt{exp}\sb\texttt{3}$} was directly created from tuples of the materialized views \textcolor{Orchid}{\texttt{prepared}}, \textcolor{Orchid}{\texttt{unprepared}} and \textcolor{Orchid}{\texttt{protein}}. It contains distinct manufacturers of products that have \textit{water} and \textit{sugar} as an ingredient, and contain \textit{protein} nutrient information; also, these manufacturers produce \textit{prepared} and \textit{unprepared} products.
    \item \textcolor{Salmon}{$\texttt{exp}\sb\texttt{4}$} was directly created from tuples of the materialized views \textcolor{CarnationPink}{$\texttt{exp}\sb\texttt{2}$} and \textcolor{Orchid}{\texttt{readytodrink}}. It contains distinct names of \texttt{readytodrink} products that contain \textit{mango} in their name, and are produced by manufacturers from the $\texttt{exp}\sb\texttt{2}$ materialized view.
\end{enumerate*}
% See Figure \ref{fig:materialized_views} for a diagram, depicting the hierarchy of our materialized views.
% \input{figures/materialized_views}
\par As stated earlier, we consider those tables that do not depend on the contents of the DB when these tables are created, and thereafter, as \textit{base tables}. Again, note that tuples can be manually inserted to and deleted from base tables, but, not in a programmatic manner over the DB, e.g., via a SQL \texttt{INSERT} statement that is based on the DB contents. In our case, the base tables are: \texttt{products}, \texttt{nutrients} and \texttt{serving\_size}. Note that each materialized view depends \textit{directly} on tuples from the base tables (as defined above) or on tuples from other previously constructed materialized views.

% Also, talk about comparing to ''related base tables'' and ''related materialized views'' during the testing, as opposed to a single table.

\subsubsection{Experiments}
% Distant Lineage and fancy stuff
\begin{runexperiment}
We test queries on a subset of the BFPDB dataset, that consists of all the tables and materialized views discussed above. In the experiments we mimic an analyst's interaction with the data by comparing the approximate lineage vectors of a target tuple with a ``heterogeneous'' group of tuples (e.g., all related base tables or all related materialized views) and ranking all the tuples among the group according to similarity scores.
\end{runexperiment}

\begin{experiment-withrun}\label{advanced-experiment:1}
We ask for distinct \texttt{manufacturers} that appear in the $\texttt{exp}\sb\texttt{3}$ materialized view, and produce products that have \textit{salt} as an ingredient:
\input{figures/q_advanced_experiment_1}
\input{tables/experiment1/base_tables_stats}
\input{tables/experiment1/base_tables_analyst-cv}
Table \ref{tab:experiment1-base-tables:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of the single result tuple in the output of this query (\textit{red gold}) against all the tuples from the related \textbf{base tables}: \texttt{products}, \texttt{nutrients} and \texttt{serving\_size}, which contain $29,322$ tuples in total. Tables \ref{tab:experiment1-base-tables:analyst-cv} and \ref{tab:experiment1-base-tables:analyst-tv} present the top 20 tuples from the related base tables, ranked by similarity, using the CV and TV methods, respectively. We make the following observations by analyzing the results:
\begin{enumerate*}
    \item The lineage sizes of the different levels (1-3) sum up to more than the total distant lineage size ($63 + 0 + 160 > 160$). In this case, it means that all 63 tuples from the $1^{st}$ lineage level (which contains tuples from the \texttt{products} relation) are also a part of the $3^{rd}$ lineage level (which contains tuples from the \texttt{products}, \texttt{nutrients} and \texttt{serving\_size} relations). From analyzing the query we conclude that these are the 63 tuples from the \texttt{products} table that affect the query result directly (via the \texttt{FROM} clause) and indirectly (via tuples from $\texttt{exp}\sb\texttt{3}$).
    % , see a path from $\texttt{exp}\sb\texttt{3}$ to \texttt{products} in Figure \ref{fig:materialized_views}
    \item The Column Vectors (CV) method demonstrates overall superiority, compared to the Tuple Vectors (TV) method. Moreover, the  CV method has a precision of 0.9 for the top $0.75\cdot160 = 120$ tuples in the approximate lineage, and 0.74 for the top 160 tuples. That is, most of the errors are produced for the lower ranked tuples (ranked 121, ..., 160).
    \item The CV method exhibits relatively high L[1] and L[3] recall scores (see Table \ref{tab:experiment1-base-tables:precision-and-recall}), evidenced by observing the Lineage Level(s) column in Table \ref{tab:experiment1-base-tables:analyst-cv}. That is, not only that all the top-20 tuples by similarity are really a part of the distant lineage, but also, the ranking preserves a level-based bias (most of the top-20 are in the $1^{st}$ lineage level). By contrast, the TV method is less impressive on this front, as is evidenced by the \textcolor{Red}{No} results in Table \ref{tab:experiment1-base-tables:analyst-tv}.
    \item Note that a random choice of the top 160 lineage tuples would have yielded a $\frac{160}{29,322} \approx 0.006$ precision score, which is several orders of magnitude worse than the scores of the CV and TV methods. 
\end{enumerate*}
\input{tables/experiment1/base_tables_analyst-tv}\input{tables/experiment3/materialized_views_stats}
% \input{tables/experiment1/base_tables_stats}

% Table \ref{tab:experiment1-materialized-views:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of the single result tuple in the output of this query (\textit{red gold}) against all the tuples from the related \textbf{materialized views}: $\texttt{exp}\sb\texttt{3}$, \texttt{protein}, \texttt{prepared} and \texttt{unprepared}, which contain $10,295$ tuples in total. Tables \ref{tab:experiment1-materialized-views:analyst-cv} and \ref{tab:experiment1-materialized-views:analyst-tv} present subsets of the top 90 and 100 (respectively) tuples from the related materialized views, ranked by similarity, using the CV and TV methods, respectively. We make some observations by analyzing the results:
% \begin{enumerate}
%     \item Both the CV and TV methods exhibit impressive outcomes, in terms of total precision and per-level recall, although the CV method performs better. That is, out of the top 85 tuples, only two are mistakenly ranked as lineage tuples (with a total of 83 tuples actually in the exact distant lineage), as can be seen in Table \ref{tab:experiment1-materialized-views:analyst-cv}.
%     \item The top rated tuple, in both methods, is the only tuple in the $1^{st}$ lineage level (from $\texttt{exp}\sb\texttt{3}$). This somewhat supports our claim of level-based bias.
%     \item The CV method showcases a significant separation between the similarity scores of the lowest ranked ``correct'' lineage tuples (up to the $85^{th}$ tuple, including) and the next non-lineage one ($0.78 > 0.67$), see Table \ref{tab:experiment1-materialized-views:analyst-cv}. On the other hand, the TV method has no evident separation at all, as can be observed in Table \ref{tab:experiment1-materialized-views:analyst-tv} (see tuples 81-100).
% \end{enumerate}

% \input{tables/experiment1/base_tables_analyst-cv}
% \input{tables/experiment1/base_tables_analyst-tv}
% \input{tables/experiment1/materialized_views_stats}
% \input{tables/experiment1/materialized_views_analyst-cv}
% \input{tables/experiment1/materialized_views_analyst-tv}
\end{experiment-withrun}


% \begin{experiment-withrun}\label{advanced-experiment:2}
% We ask for distinct pairs of (\texttt{manufacturer}, \texttt{name}) for products that are listed in the $\texttt{exp}\sb\texttt{4}$ materialized view:\footnotemark
% \input{figures/q_advanced_experiment_2}
% \footnotetext{For a detailed description of $\texttt{exp}\sb\texttt{4}$ see section \ref{appendix:sec:exp4} in the appendix.}

% Table \ref{tab:experiment2-base-tables:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of the (two) result tuples in the output of this query ((\textit{campbell soup company, v8 beverage carrot mango}), (\textit{campbell soup company, v8 vfusion beverage peach mango})) against all the tuples from the related \textbf{base tables}: \texttt{products}, \texttt{nutrients} and \texttt{serving\_size}, which contain $29,322$ tuples in total. Tables \ref{tab:experiment2-base-tables:analyst-cv} and \ref{tab:experiment2-base-tables:analyst-tv} present the top 20 tuples from the related base tables, ranked by similarity to result tuple No.\texttt{0}, using the CV and TV methods, respectively. We make some observations by analyzing the results:
% \begin{enumerate}
%     \item The lineage sizes (of both result tuples) of the different levels (1-4) sum up to more than the total distant lineage sizes. E.g., looking at result tuple No.\texttt{0}: $2 + 0 + 4 + 80 > 82$. In this case, it means that at least two of the four tuples from the $3^{rd}$ lineage level (which contains tuples from the \texttt{products} and \texttt{serving\_size} relations, via $\texttt{exp}\sb\texttt{4}\longrightarrow\texttt{readytodrink}$, see Figure \ref{fig:materialized_views}) are also a part of either the $1^{st}$ lineage level (which contains tuples from the \texttt{products} relation, via the \texttt{FROM} clause), or the $4^{th}$ lineage level (which contains tuples from the \texttt{products}, \texttt{nutrients} and \texttt{serving\_size} relations).
%     \item The Column Vectors (CV) method demonstrates overall superiority, compared to the Tuple Vectors (TV) method, topping at a precision score of 0.81 for the top 82 (total lineage size) approximate lineage tuples, for both result tuples.  Moreover, the TV method demonstrates unusually low  ($\approx0.2$) precision scores for this query.
%     \item The TV method exhibits perfect L[1] and L[3] recall scores, and a low L[4] recall score, for both result tuples (see Table \ref{tab:experiment2-base-tables:precision-and-recall}). We conclude that the TV method is highly effective in finding the $1^{st}$ and $3^{rd}$ lineage-level tuples, but performs poorly in finding the $4^{th}$ lineage-level tuples, as is evidenced by the \textcolor{Red}{No} results in Table \ref{tab:experiment2-base-tables:analyst-tv}.
%     \item The CV method exhibits relatively high L[1] and L[4] recall scores and a somewhat mediocre L[3] recall score for both result tuples (see Table \ref{tab:experiment2-base-tables:precision-and-recall}), evidenced by observing the Lineage Level(s) column in Table \ref{tab:experiment2-base-tables:analyst-cv}. That is, not only that almost all the top-20 tuples by similarity are really a part of the distant lineage, but also, the ranking preserves a level-based bias (the top-2 tuples are the only ones that appear both in the $1^{st}$, $3^{rd}$ and $4^{th}$ lineage levels).
%     \item Analyzing the Tables \ref{tab:experiment2-base-tables:analyst-cv} and \ref{tab:experiment2-base-tables:analyst-tv}, we see that the two $3^{rd}$ lineage-level tuples from the \texttt{serving\_size} relation are discovered significantly earlier in the ranking by the TV method ($3^{rd}$ and $4^{th}$ tuples, by similarity) in comparison with the CV method ($80^{th}$ and $83^{rd}$ tuples, by similarity). This means that the TV method does a better job on the $3^{rd}$ lineage level, in terms of recall. This observation is backed up by the L[3] recall results we see in Table \ref{tab:experiment2-base-tables:precision-and-recall}.
%     \item Notice the $4^{th}$ ranked tuple (by similarity) in Table \ref{tab:experiment2-base-tables:analyst-cv}, which is a \textcolor{Red}{No} lineage tuple, with a relatively high similarity score. A closer look reveals that this tuple is a product named \textit{v8 splash beverage mango peach}, which is also produced by \textit{campbell soup company}. Interestingly, it also appears as the first \textcolor{Red}{No} tuple when analyzing result tuple No.\texttt{1} vs. related base tables with the CV method (we do not show this explicitly).
%     \item Note that a random choice of the top 82 lineage tuples would have yielded a $\frac{82}{29,322} \approx 0.003$ precision score, which is several orders of magnitude worse than the scores of the CV (and even the TV) methods. 
% \end{enumerate}

% \input{tables/experiment2/base_tables_stats}

% Table \ref{tab:experiment2-materialized-views:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of the (two) result tuples in the output of this query ((\textit{campbell soup company, v8 beverage carrot mango}), (\textit{campbell soup company, v8 vfusion beverage peach mango})) against all the tuples from the related \textbf{materialized views}: $\texttt{exp}\sb\texttt{4}$, $\texttt{exp}\sb\texttt{2}$, \texttt{protein}, \texttt{unprepared} and \texttt{readytodrink}, which contain $9,658$ tuples in total. Tables \ref{tab:experiment2-materialized-views:analyst-cv} and \ref{tab:experiment2-materialized-views:analyst-tv} present the top 20 tuples from the related materialized views, ranked by similarity to result tuple No.\texttt{0}, using the CV and TV methods, respectively. We make some observations by analyzing the results:
% \begin{enumerate}
%     \item The CV method demonstrates overall superiority, compared to the TV method, in terms of total precision and per-level recall. For example, for result tuple No.\texttt{0}, out of the top 44 tuples, only four are mistakenly ranked as lineage tuples (with a total of 40 tuples actually in the exact distant lineage), as can be partially seen in Table \ref{tab:experiment2-materialized-views:analyst-cv}.
%     \item The top rated tuple in the CV method (Table \ref{tab:experiment2-materialized-views:analyst-cv}), is the only tuple in the $1^{st}$ lineage level (from $\texttt{exp}\sb\texttt{4}$). This somewhat supports our claim of level-based bias (the L[2] and L[3] recall scores are relatively high as well).
%     \item By contrast, for result tuple No.\texttt{0}, the TV method ranks the only $1^{st}$ lineage-level tuple from $\texttt{exp}\sb\texttt{4}$ in $3^{rd}$ place, which is evidenced by the 0\footnotemark\, L[1] score in Table \ref{tab:experiment2-materialized-views:precision-and-recall} and can be seen in detail in Table \ref{tab:experiment2-materialized-views:analyst-tv}.
%     \footnotetext{Following the definitions in section \ref{sec:recall}:\\
%     $\operatorname{Recall}(t_0, 1) = \frac{|ApproxLineage(t_0, D(t_0, 1)) \cap L_{t_0}[1])|}{|L_{t_0}[1]|} = \frac{|ApproxLineage(t_0, |L_{t_0}[1]|) \cap L_{t_0}[1])|}{|L_{t_0}[1]|} = \frac{|ApproxLineage(t_0, 1) \cap L_{t_0}[1])|}{1} = |\{t_{\texttt{protein}}\} \cap \{t_{\texttt{$\texttt{exp}\sb\texttt{4}$}}\}| = |\emptyset| = 0$}
%     \item Both the TV and CV methods rank the other, non-lineage tuple from $\texttt{exp}\sb\texttt{4}$, in the top 20, without a significant similarity score separation between the correct and the incorrect tuples from $\texttt{exp}\sb\texttt{4}$ (0.99 vs. 0.94 for the CV method, and 0.96 vs. 0.9 for the TV method). This suggests a relatively high similarity in terms of lineage, between the two tuples in the $\texttt{exp}\sb\texttt{4}$ materialized view (from transitivity).
% \end{enumerate}

% \input{tables/experiment2/base_tables_analyst-cv}
% \input{tables/experiment2/base_tables_analyst-tv}
% \input{tables/experiment2/materialized_views_stats}
% \input{tables/experiment2/materialized_views_analyst-cv}
% \input{tables/experiment2/materialized_views_analyst-tv}
% \end{experiment-withrun}

% \input{tables/experiment3/materialized_views_stats}
\begin{experiment-withrun}\label{advanced-experiment:3}
We ask for distinct pairs of (\texttt{manufacturer}, \texttt{name}) for products from the \texttt{sugars} materialized view, that contain \textit{rice} in their name, and are produced by manufacturers that appear in the $\texttt{exp}\sb\texttt{2}$ materialized view:
\input{figures/q_advanced_experiment_3}

% Table \ref{tab:experiment3-base-tables:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of four (out of nine, for brevity) of the result tuples in the output of this query against all the tuples from the related \textbf{base tables}: \texttt{products}, \texttt{nutrients} and \texttt{serving\_size}, which contain $29,322$ tuples in total. Tables \ref{tab:experiment3-base-tables:analyst-cv} and \ref{tab:experiment3-base-tables:analyst-tv} present subsets of the top 100 and 20 (respectively) tuples from the related base tables, ranked by similarity to result tuple No.\texttt{2}, using the CV and TV methods, respectively. We make some observations by analyzing the results:
% \begin{enumerate}
%     \item This query presents a case where the size of the total distant lineage of result tuples is significant in terms of the input DB size. E.g., the total distant lineage size of result tuple No.\texttt{2} is $4,000$, while the related base tables contain a total of $29,322$ tuples ($\approx 1:10$).
%     \item The Column Vectors (CV) method demonstrates overall superiority, compared to the Tuple Vectors (TV) method. Moreover, analyzing result tuple No.\texttt{2}, the CV method has a precision of 0.97 for the top $0.5\cdot4,000 = 2,000$ tuples in the approximate lineage, and 0.67 for the top $4,000$ tuples. That is, most of the errors are produced for the lower ranked tuples (ranked 2001, ..., 4000). These numbers are shown explicitly in Table \ref{tab:experiment3-base-tables:analyst-cv}, that shows the $52^{nd}$ ranked tuple as the only non-lineage tuple in the top 100.
%     \item The TV method exhibits perfect L[1] and L[2] recall scores, and a low L[3] recall score, for all four result tuples (see Table \ref{tab:experiment3-base-tables:precision-and-recall}). We conclude that the TV method is highly effective in finding the $1^{st}$ and $2^{nd}$ lineage-level tuples, but performs poorly in finding the $3^{rd}$ lineage-level tuples, as is evidenced by the \textcolor{Red}{No} results in Table \ref{tab:experiment3-base-tables:analyst-tv}.
%     \item The CV method exhibits perfect L[1] recall scores and relatively high L[2] and L[3] recall scores (see Table \ref{tab:experiment3-base-tables:precision-and-recall}). Analyzing result tuple No.\texttt{2} and Table \ref{tab:experiment3-base-tables:analyst-cv}, the 0.5 L[2] recall score seems a little misleading, since the $2^{nd}$ L[2] lineage-level tuple is not ``lost'', but is ranked $3^{rd}$ (instead of $2^{nd}$). This somewhat supports our claim of level-based bias.
%     \item Note that a random choice of the top $4,000$ lineage tuples would have yielded a $\frac{4,000}{29,322} \approx 0.136$ precision score, which is comparable with the scores of the TV method, but, is significantly worse than the CV method scores.
% \end{enumerate}

% \input{tables/experiment3/base_tables_stats}
% \input{tables/experiment3/materialized_views_stats}
\input{tables/experiment3/materialized_views_analyst-cv}
\input{tables/experiment3/materialized_views_analyst-tv}

Table \ref{tab:experiment3-materialized-views:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of four (out of nine, for brevity) of the result tuples in the output of this query against all the tuples from the related \textbf{materialized views}: $\texttt{exp}\sb\texttt{2}$, \texttt{protein}, \texttt{sugars} and \texttt{unprepared}, which contain $10,298$ tuples in total. Tables \ref{tab:experiment3-materialized-views:analyst-cv} and \ref{tab:experiment3-materialized-views:analyst-tv} present the top 15 tuples from the related materialized views, ranked by similarity to result tuple No.\texttt{2}, using the CV and TV methods, respectively. We make the following observations by analyzing the results:
\begin{enumerate*}
    \item Once again, the CV method demonstrates overall superiority, compared to the TV method, in terms of total precision and per-level recall.
    \item Analyzing result tuple No.\texttt{2}, the top rated tuple in both the CV and TV methods (see Tables \ref{tab:experiment3-materialized-views:analyst-cv} and \ref{tab:experiment3-materialized-views:analyst-tv}, respectively) is the only \texttt{sugars} tuple in the $1^{st}$ lineage level. The $2^{nd}$ tuple in the $1^{st}$ (L[1]) lineage level (from $\texttt{exp}\sb\texttt{2}$) is ``discovered'' earlier (ranked $3^{rd}$ vs. $5^{th}$) in the CV method, with no similarity score separation from the higher ranked tuples. By contrast, the TV method exhibits a significant similarity score drop all across the top 15 ranked tuples (0.97 for $1^{st}$ ranked vs. 0.81 for $5^{th}$ ranked vs. 0.65 for $15^{th}$ ranked). We view a more stable similarity score progression as indicating a better overall performance.
    \item Analyzing Tables \ref{tab:experiment3-materialized-views:precision-and-recall} and \ref{tab:experiment3-materialized-views:analyst-cv}, it seems the numbers for result No.\texttt{2} are not as good (compared to previous experiments and the result tuples No.\texttt{0} and No.\texttt{1} in this current experiment). A closer look reveals that out of the top 100 ranked tuples (by similarity) - all the mistakes are made on tuples from the \texttt{sugars} and \texttt{protein} materialized views. The \textcolor{Red}{No} tuples from \texttt{sugars} and \texttt{protein} are mostly products that appear also in the \texttt{unprepared} materialized view, and are actually in the lineage (i.e., \textcolor{Green}{Yes} tuples) of result tuple No.\texttt{2}. It seems that these \textcolor{Red}{No} tuples from \texttt{sugars} and \texttt{protein} have the same lineage vectors per the product related columns as the respective \textcolor{Green}{Yes} tuples from \texttt{unprepared}. Now, the Query Dependency DAG has no real filtering capabilities in this case (since the queries that created \texttt{sugars} and \texttt{protein} are relevant), hence we are not able to effectively eliminate these mistakes.

\end{enumerate*}
% \input{tables/experiment3/materialized_views_analyst-cv}
% \input{tables/experiment3/materialized_views_analyst-tv}

% \input{tables/experiment3/base_tables_analyst-cv}
% \input{tables/experiment3/base_tables_analyst-tv}
% \input{tables/experiment3/materialized_views_stats}
% \input{tables/experiment3/materialized_views_analyst-cv}
% \input{tables/experiment3/materialized_views_analyst-tv}
\end{experiment-withrun}




\begin{experiment-withrun}\label{advanced-experiment:2}
We ask for distinct pairs of (\texttt{manufacturer}, \texttt{name}) for products that are listed in the $\texttt{exp}\sb\texttt{4}$ materialized view:
\input{figures/q_advanced_experiment_2}
\input{tables/experiment2/base_tables_stats}

Table \ref{tab:experiment2-base-tables:precision-and-recall} presents lineage related statistics, collected when computing the approximate lineage of the (two) result tuples in the output of this query ((\textit{campbell soup company, v8 beverage carrot mango}), (\textit{campbell soup company, v8 vfusion beverage peach mango})) against all the tuples from the related \textbf{base tables}: \texttt{products}, \texttt{nutrients} and \texttt{serving\_size}, which contain $29,322$ tuples in total. Tables \ref{tab:experiment2-base-tables:analyst-cv} and \ref{tab:experiment2-base-tables:analyst-tv} present a subset of the top 83 tuples from the related base tables, ranked by similarity to result tuple No.\texttt{0}, using the CV and TV methods, respectively. We make the following observations by analyzing the results:
\begin{enumerate*}
    \item The lineage sizes (of both result tuples) of the different levels (1-4) sum up to more than the total distant lineage sizes. E.g., looking at result tuple No.\texttt{0}: $2 + 0 + 4 + 80 > 82$. In this case, it means that at least two of the four tuples from the $3^{rd}$ lineage level (which contains tuples from the \texttt{products} and \texttt{serving\_size} relations) are also a part of either the $1^{st}$ lineage level (which contains tuples from the \texttt{products} relation), or the $4^{th}$ lineage level (which contains tuples from the \texttt{products}, \texttt{nutrients} and \texttt{serving\_size} relations).
    \item The Column Vectors (CV) method demonstrates overall superiority, compared to the Tuple Vectors (TV) method, topping at a precision score of 0.81 for the top 82 (total lineage size) approximate lineage tuples, for both result tuples.  Moreover, the TV method demonstrates unusually low  ($\approx0.2$) precision scores for this query.
    \item The TV method exhibits perfect L[1] and L[3] recall scores, and a low L[4] recall score, for both result tuples (see Table \ref{tab:experiment2-base-tables:precision-and-recall}). We conclude that the TV method is highly effective in finding the $1^{st}$ and $3^{rd}$ lineage-level tuples, but performs poorly in finding the $4^{th}$ lineage-level tuples, as is evidenced by the \textcolor{Red}{No} results in Table \ref{tab:experiment2-base-tables:analyst-tv}.
    \item The CV method exhibits relatively high L[1] and L[4] recall scores and a somewhat mediocre L[3] recall score for both result tuples (see Table \ref{tab:experiment2-base-tables:precision-and-recall}), evidenced by observing the Lineage Level(s) column in Table \ref{tab:experiment2-base-tables:analyst-cv}. That is, not only that almost all the top-20 tuples by similarity are really a part of the distant lineage, but also, the ranking preserves a level-based bias (the top-2 tuples are the only ones that appear both in the $1^{st}$, $3^{rd}$ and $4^{th}$ lineage levels).
    \item Analyzing the Tables \ref{tab:experiment2-base-tables:analyst-cv} and \ref{tab:experiment2-base-tables:analyst-tv}, we see that the two $3^{rd}$ lineage-level tuples from the \texttt{serving\_size} relation are discovered significantly earlier in the ranking by the TV method ($3^{rd}$ and $4^{th}$ tuples, by similarity) in comparison with the CV method ($80^{th}$ and $83^{rd}$ tuples, by similarity). This means that the TV method does a better job on the $3^{rd}$ lineage level, in terms of recall. This observation is backed up by the L[3] recall results we see in Table \ref{tab:experiment2-base-tables:precision-and-recall}.
    \item Notice the $4^{th}$ ranked tuple (by similarity) in Table \ref{tab:experiment2-base-tables:analyst-cv}, which is a \textcolor{Red}{No} lineage tuple, with a relatively high similarity score. A closer look reveals that this tuple is a product named \textit{v8 splash beverage mango peach}, which is also produced by \textit{campbell soup company}. Interestingly, it also appears as the first \textcolor{Red}{No} tuple when analyzing result tuple No.\texttt{1} vs. related base tables with the CV method (we do not show this explicitly).
    \item Note that a random choice of the top 82 lineage tuples would have yielded a $\frac{82}{29,322} \approx 0.003$ precision score, which is several orders of magnitude worse than the scores of the CV (and even the TV) methods. 
\end{enumerate*}

% \input{tables/experiment2/base_tables_stats}
\input{tables/experiment2/base_tables_analyst-cv}
\input{tables/experiment2/base_tables_analyst-tv}

\end{experiment-withrun}


==> main/discussion.tex <==
\chapter{Discussion}
\label{chap:discussion}


% % Relational Embeddings
% \section{Relational embedding} is a very active area of research \cite{DBLP:journals/corr/abs-1803-01384, sigmod2020_keynote, pie2020_keynote}.
% When converting a relational DB to unstructured text (see section \ref{sec:latent_wv_model}) special care is required to support numerical values correctly. Bordawekar and Shmueli \cite{DBLP:journals/corr/BordawekarS16} take the route of tokenizing numerical values from the DB by preceding each number with a ``range designator'' (e.g., 1-10, 50-100, SMALL, BIG, etc.) in the generated corpus. In \cite{DBLP:journals/corr/abs-1712-07199} Bordawekar, Bandyopadhyay and Shmueli use clustering techniques to represent numerical values textually. In contrast, in this work we deal with numerical values by concatenating the relevant column name to each number in the generated corpus. This way, we ensure our model separates between numerical values of different fields, as they are conceptually different, semantically speaking (for example, we want the value 300 for a \texttt{nutrient\_code} field in a \texttt{nutrients} table to have a different learned vector than the value 300 for a \texttt{household\_serving\_size} field in a \texttt{serving\_size} table, from the USDA BFPDB dataset). 

% Following up on section \ref{sec:latent_wv_model} it should be noted that we train word embeddings for both textual and numerical columns and values, when . Numeric types for example require special care during training (we draw inspiration from the work on CI Queries of Bordawekar and Shmueli \cite{DBLP:journals/corr/BordawekarS16}; they use the term \textit{db2vec}). The distinction in strategy between different data types is done only in the preparation step to training the word embeddings model. 

% % Provenance Vectors
% Following up on section \ref{sec:proposed_solution_approx} we would like to clarify the intended usage of the \textbf{lineage vectors}. When using tuple-based provenance vectors:
% \begin{itemize}
%     \item Each manually inserted tuple - has a set of 1 tuple vectors.
%     \item Each tuple in the result of a query - has a set of up to $max\_vectors\_num$ tuple vectors.
%     \item We always compare between two sets of tuple vectors using the formula in section \ref{sec:latent_wv_model}.
% \end{itemize}
% When using column-based provenance vectors:
% \begin{itemize}
%     \item Analogous to tuple vectors but everything is done at the column level (see section \ref{sec:column-vectors}).
% \end{itemize}

% % Bloom Filters and timestamps
% \section{Bloom-Filters and Timestamps} Bloom-Filters and timestamps are universal enhancements that can be applied to any lineage-approximation technique. They complement beautifully the word embedding based lineage vectors, but are far from being a ``silver bullet'' on their own.
% In particular, in the extreme case where most (or even all) the tuples of a table \texttt{A} participated in the evaluation of a query $q$, the Bloom Filters (almost) will not help when comparing a tuple from the result of $q$ to tuples from table \texttt{A}.

% % Natural Ranking
% \section{A Natural Ranking of Explanations}
% Our method implicitly produces a ``natural ranking'' of explanations. It is unclear how to get this kind of ranking from semiring provenance polynomials (it might require significant additional manual work). To this end, there is a work by Deutch et al. \cite{Deutch2015} that ranks derivation trees for Datalog programs. In contrast, we deal with simpler SQL queries and we look at a much simpler notion: lineage, providing a succinct good-enough and useful one.

==> tables/bfpdb_samples/nutrients.tex <==
\begin{table}[H]
% \centering
% \begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    format index, format samples-table, format samples-nutrients,
    col sep=comma,
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     {ndb-no}, {nutrient-code},  {nutrient-name},  {derivation-code}     , {out-val}, {out-uom}           
    0,     45127286,            301,          calcium ca,                  lccd     , 1      ,  123
    1,     45375142,            307,          sodium na,                  lcsa , 1, 1
    2,     45375117,            601,          cholesterol,                  lccd , 1, 1
    3,     45375228,            269,          sugars total,                  lcsa   , 1,  1
    4,     45321384,            605,          fatty acids total trans,                  lcsa    , 1, 1
}
% \end{adjustbox}
% \textbf{\caption{\label{tab:bpfdb_samples:nutrients}
%                 }
%         }
\end{table}

==> tables/bfpdb_samples/products.tex <==
\begin{table}[H]
\centering
% \begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    format index, format samples-table, format samples-nutrients,
    col sep=comma,
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     {ndb-no}, {nutrient-code},  {nutrient-name},  {derivation-code}                
    0,     45127286,            301,          calcium ca,                  lccd 
    1,     45375142,            307,          sodium na,                  lcsa
    2,     45375117,            601,          cholesterol,                  lccd 
    3,     45375228,            269,          sugars total,                  lcsa     
    4,     45321384,            605,          fatty acids total trans,                  lcsa
}
% \end{adjustbox}
% \textbf{\caption{\label{tab:bpfdb_samples:nutrients}
%                 }
%         }
\end{table}

==> tables/experiment1/materialized_views_analyst-cv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.55,max=0.98, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    $\texttt{exp}\sb\texttt{3}$,    0.975,    {1}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    protein,     0.939,    {2}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    protein,    0.937,    {2}          ,\textcolor{Green}{Yes}
    3,     $id_4$,    protein,    0.936,    {2}          ,\textcolor{Green}{Yes}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    17,     $id_{18}$,    unprepared,    0.922,    {2}          ,\textcolor{Green}{Yes}
    18,     $id_{19}$,    unprepared,    0.920,    {2}          ,\textcolor{Green}{Yes}
    19,     $id_{20}$,    unprepared,    0.917,    {2}          ,\textcolor{Green}{Yes}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    80,     $id_{81}$,    unprepared,    0.833,    {2}          ,\textcolor{Green}{Yes}
    81,     $id_{82}$,    unprepared,    0.827,    {2}          ,\textcolor{Green}{Yes}
    82,     $id_{83}$,    unprepared,   0.825,    {2}          ,\textcolor{Green}{Yes}
    83,     $id_{84}$,    unprepared,    0.817,    {2}          ,\textcolor{Green}{Yes}
    84,     $id_{85}$,    unprepared,    0.775,    {2}          ,\textcolor{Green}{Yes}
    85,     $id_{86}$,    unprepared,    0.670,              ,\textcolor{Red}{No}
    86,     $id_{87}$,    unprepared,    0.668,              ,\textcolor{Red}{No}
    87,     $id_{88}$,    unprepared,    0.667,              ,\textcolor{Red}{No}
    88,     $id_{89}$,    unprepared,    0.664,              ,\textcolor{Red}{No}
    89,     $id_{90}$,    unprepared,    0.664,              ,\textcolor{Red}{No}


}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment1-materialized-views:analyst-cv}
                Experiment \ref{advanced-experiment:1} \textit{red gold} vs. related \textbf{materialized views} with \textbf{Column Vectors} - an analyst's view.
                A subset of the top-90 tuples from the related materialized views, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Column Vectors method.
                }
        }
\end{table}

==> tables/experiment1/materialized_views_analyst-tv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.55,max=0.98, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    $\texttt{exp}\sb\texttt{3}$,    0.937,    {1}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    unprepared,     0.866,    {2}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    unprepared,    0.860,    {2}          ,\textcolor{Green}{Yes}
    3,     $id_4$,    unprepared,    0.858,    {2}          ,\textcolor{Green}{Yes}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    17,     $id_{18}$,    unprepared,    0.761,    {2}          ,\textcolor{Green}{Yes}
    18,     $id_{19}$,    unprepared,    0.760,    {2}          ,\textcolor{Green}{Yes}
    19,     $id_{20}$,    unprepared,    0.760,    {2}          ,\textcolor{Green}{Yes}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    80,     $id_{81}$,    unprepared,    0.674,              ,\textcolor{Red}{No}
    81,     $id_{82}$,    unprepared,    0.674,    {2}          ,\textcolor{Green}{Yes}
    82,     $id_{83}$,    unprepared,   0.673,              ,\textcolor{Red}{No}
    83,     $id_{84}$,    unprepared,    0.672,     {2}         ,\textcolor{Green}{Yes}
    84,     $id_{85}$,    unprepared,    0.671,    {2}          ,\textcolor{Green}{Yes}
    85,     $id_{86}$,    unprepared,   0.667,      {2}        ,\textcolor{Green}{Yes}
    86,     $id_{87}$,    unprepared,    0.667,     {2}         ,\textcolor{Green}{Yes}
    87,     $id_{88}$,    unprepared,    0.667,    {2}          ,\textcolor{Green}{Yes}
    88,     $id_{89}$,    unprepared,   0.666,      {2}        ,\textcolor{Green}{Yes}
    89,     $id_{90}$,    unprepared,    0.663,    {2}          ,\textcolor{Green}{Yes}
    90,     $id_{91}$,    unprepared,    0.662,     {2}         ,\textcolor{Green}{Yes}
    91,     $id_{92}$,    unprepared,    0.662,              ,\textcolor{Red}{No}
    92,     $id_{93}$,    unprepared,    0.662,             ,\textcolor{Red}{No}
    93,     $id_{94}$,    unprepared,    0.660,         {2}     ,\textcolor{Green}{Yes}
    94,     $id_{95}$,    unprepared,    0.660,              ,\textcolor{Red}{No}
    95,     $id_{96}$,    unprepared,    0.659,              ,\textcolor{Red}{No}
    96,     $id_{97}$,    unprepared,    0.657,              ,\textcolor{Red}{No}
    97,     $id_{98}$,    unprepared,    0.657,              ,\textcolor{Red}{No}
    98,     $id_{99}$,    unprepared,    0.656,              ,\textcolor{Red}{No}
    99,     $id_{100}$,    unprepared,    0.655,              ,\textcolor{Red}{No}


}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment1-materialized-views:analyst-tv}
                Experiment \ref{advanced-experiment:1} \textit{red gold} vs. related \textbf{materialized views} with \textbf{Tuple Vectors} - an analyst's view.
                A subset of the top-100 tuples from the related materialized views, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Tuple Vectors method.
                }
        }
\end{table}

==> tables/experiment1/materialized_views_stats.tex <==
\begin{table*}
\centering
\begin{adjustbox}{width=\textwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.32,max=1.0}, format index, format stats-table2-exp1, format manufacturer, format method,
    col sep=comma,
    /pgfplots/colormap={orange}{
        rgb255(0cm)=(255,245,235);
        rgb255(1cm)=(253,141,60)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    
    index,  Provenance Method,       manufacturer, Total, Length-L1, Length-L2, Length-L3,  {1.00$^{Top}$},            {0.75$^{Top}$},        {0.50$^{Top}$},        {0.25$^{Top}$}, Recall-L1, Recall-L2  
    0,      Tuple Vectors,   red gold, 83, 1, 82, 0,     0.831 ,        0.873 ,     0.952 ,       0.952, 1.0, 0.829
    1,      Column Vectors,   red gold, 83, 1, 82, 0,    0.964 ,        0.952 ,     0.929 ,       0.952, 1.0, 0.963
}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment1-materialized-views:precision-and-recall}
                Experiment \ref{advanced-experiment:1} \textit{red gold} vs. materialized views ($\texttt{exp}\sb\texttt{3}$, \texttt{protein}, \texttt{prepared} and \texttt{unprepared}).
                A comparison of different approximate lineage computation methods on a single query-result tuple (\textit{red gold}). Total Lineage Size is the size of the exact distant lineage for a result tuple (containing only tuples from the related materialized views). Similarly, L[$i$] is the size of the $i^{th}$ lineage level. $p^{Top}$ Precision shows the precision of various methods for the top $p\cdot|Total Distant Lineage|$ tuples in the approximate lineage. For example, 0.50$^{Top}$ is the precision for the top 41 ($=\floor{0.5\cdot83}$) tuples in the approximate lineage. L[$i$] Recall shows the $i^{th}$ lineage level recall as described in section \ref{sec:recall}.
                }
        }
\end{table*}

==> tables/experiment2/materialized_views_analyst-cv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.55,max=0.99, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    $\texttt{exp}\sb\texttt{4}$,    0.986,    {1}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    readytodrink,     0.983,    {2}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    readytodrink,    0.981,    {2}          ,\textcolor{Green}{Yes}
    3,     $id_4$,    protein,    0.971,        {3}      ,\textcolor{Green}{Yes}
    4,     $id_5$,    protein,    0.968,    {3}          ,\textcolor{Green}{Yes}
    5,     $id_6$,    $\texttt{exp}\sb\texttt{2}$,    0.965,    {2}         ,\textcolor{Green}{Yes}
    6,     $id_7$,    protein,    0.944,    {3}         ,\textcolor{Green}{Yes}
    7,     $id_8$,    unprepared,    0.944,    {3}          ,\textcolor{Green}{Yes}
    8,     $id_9$,    protein,    0.940,    {3}       ,\textcolor{Green}{Yes}
    9,     $id_{10}$,    protein,    0.939,    {3}          ,\textcolor{Green}{Yes}
    10,     $id_{11}$,    protein,    0.938,    {3}          ,\textcolor{Green}{Yes}
    11,     $id_{12}$,    protein,   0.938,    {3}         ,\textcolor{Green}{Yes}
    12,     $id_{13}$,    protein,    0.938,    {3}          ,\textcolor{Green}{Yes}
    13,     $id_{14}$,    protein,    0.938,    {3}         ,\textcolor{Green}{Yes}
    14,     $id_{15}$,    protein,    0.937,    {3}          ,\textcolor{Green}{Yes}
    15,     $id_{16}$,    protein,    0.936,      {3}        ,\textcolor{Green}{Yes}
    16,     $id_{17}$,    $\texttt{exp}\sb\texttt{4}$,    0.936,    ,\textcolor{Red}{No}
    17,     $id_{18}$,    protein,    0.935,    {3}          ,\textcolor{Green}{Yes}
    18,     $id_{19}$,    protein,    0.933,    {3}          ,\textcolor{Green}{Yes}
    19,     $id_{20}$,    protein,    0.932,    {3}          ,\textcolor{Green}{Yes}


}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment2-materialized-views:analyst-cv}
                Experiment \ref{advanced-experiment:2} result tuple No.\texttt{0} vs. related \textbf{materialized views} with \textbf{Column Vectors} - an analyst's view.
                Top-20 tuples from the related base tables, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Column Vectors method.
                }
        }
\end{table}

==> tables/experiment2/materialized_views_analyst-tv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.55,max=0.98, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    protein,    0.967,    {3}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    readytodrink,     0.964,    {2}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    $\texttt{exp}\sb\texttt{4}$,    0.960,    {1}          ,\textcolor{Green}{Yes}
    3,     $id_4$,    protein,    0.957,        {3}      ,\textcolor{Green}{Yes}
    4,     $id_5$,    readytodrink,    0.956,    {2}          ,\textcolor{Green}{Yes}
    5,     $id_6$,    $\texttt{exp}\sb\texttt{2}$,    0.905,    {2}         ,\textcolor{Green}{Yes}
    6,     $id_7$,    $\texttt{exp}\sb\texttt{4}$,    0.899,             ,\textcolor{Red}{No}
    7,     $id_8$,    protein,    0.767,   {3}           ,\textcolor{Green}{Yes}
    8,     $id_9$,    readytodrink,    0.754,           ,\textcolor{Red}{No}
    9,     $id_{10}$,    readytodrink,    0.752,              ,\textcolor{Red}{No}
    10,     $id_{11}$,    readytodrink,    0.749,              ,\textcolor{Red}{No}
    11,     $id_{12}$,    readytodrink,   0.747,             ,\textcolor{Red}{No}
    12,     $id_{13}$,    protein,    0.741,    {3}          ,\textcolor{Green}{Yes}
    13,     $id_{14}$,    readytodrink,    0.739,             ,\textcolor{Red}{No}
    14,     $id_{15}$,    readytodrink,    0.735,              ,\textcolor{Red}{No}
    15,     $id_{16}$,    protein,    0.725,      {3}        ,\textcolor{Green}{Yes}
    16,     $id_{17}$,    protein,    0.724,  {3}   ,\textcolor{Green}{Yes}
    17,     $id_{18}$,    protein,    0.724,    {3}          ,\textcolor{Green}{Yes}
    18,     $id_{19}$,    readytodrink,    0.722,              ,\textcolor{Red}{No}
    19,     $id_{20}$,    protein,    0.721,    {3}          ,\textcolor{Green}{Yes}


}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment2-materialized-views:analyst-tv}
                Experiment \ref{advanced-experiment:2} result tuple No.\texttt{0} vs. related \textbf{materialized views} with \textbf{Tuple Vectors} - an analyst's view.
                Top-20 tuples from the related base tables, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Tuple Vectors method.
                }
        }
\end{table}

==> tables/experiment2/materialized_views_stats.tex <==
\begin{table*}
\centering
\begin{adjustbox}{width=\textwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.32,max=1.0}, format index, format stats-table2-exp2, format manufacturer, format method,
    col sep=comma,
    /pgfplots/colormap={orange}{
        rgb255(0cm)=(255,245,235);
        rgb255(1cm)=(253,141,60)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    
    index,  Provenance Method,       manufacturer, name, Total, Length-L1, Length-L2, Length-L3, Length-L4,  {1.00$^{Top}$},            {0.75$^{Top}$},        {0.50$^{Top}$},        {0.25$^{Top}$}, Recall-L1, Recall-L2, Recall-L3
    0, Tuple Vectors, campbell soup company, v8 beverage carrot mango, 44, 1, 3, 40, 0, 0.5, 0.5, 0.609, 0.583, 0, 0.333, 0.450
    1, , campbell soup company, v8 vfusion beverage peach mango, 44, 1, 3, 40, 0, 0.545, 0.529, 0.609, 0.583, 1, 0.667, 0.5
    0, Column Vectors, campbell soup company, v8 beverage carrot mango, 44, 1, 3, 40, 0, 0.909, 0.912, 0.957, 1, 1, 0.667, 0.900
    1, , campbell soup company, v8 vfusion beverage peach mango, 44, 1, 3, 40, 0, 0.773, 0.824, 0.957, 0.917, 1, 0.667, 0.750
}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment2-materialized-views:precision-and-recall}
                Experiment \ref{advanced-experiment:2} query results vs. related materialized views ($\texttt{exp}\sb\texttt{2}$, \texttt{protein}, \texttt{unprepared} and \texttt{readytodrink}).
                A comparison of different approximate lineage computation methods on the query-result tuples. Total Lineage Size is the size of the exact distant lineage for a result tuple (containing only tuples from the related materialized views). Similarly, L[$i$] Lineage Size is the size of the $i^{th}$ lineage level. $p^{Top}$ Precision shows the precision of various methods for the top $p\cdot|Total Distant Lineage|$ tuples in the approximate lineage. For example, 0.50$^{Top}$ is the precision for the top 21 ($=0.5\cdot43$) tuples in the approximate lineage. L[$i$] Recall shows the $i^{th}$ lineage level recall as described in section \ref{sec:recall}.
                }
        }
\end{table*}

==> tables/experiment3/base_tables_analyst-cv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.7,max=0.9, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    products,    0.994,    {1, 2, 3}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    products,     0.993,    {3}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    products,    0.963,    {2}          ,\textcolor{Green}{Yes}
    3,     $id_4$,    products,    0.954,     {3}         ,\textcolor{Green}{Yes}
    4,     $id_5$,    products,    0.953,    {3}          ,\textcolor{Green}{Yes}
    5,     $id_6$,    products,    0.951,    {3}        ,\textcolor{Green}{Yes}
    6,     $id_7$,    products,    0.947,    {3}         ,\textcolor{Green}{Yes}
    7,     $id_8$,    nutrients,    0.947,    {3}          ,\textcolor{Green}{Yes}
    8,     $id_9$,    products,    0.945,    {3}       ,\textcolor{Green}{Yes}
    9,     $id_{10}$,    products,    0.945,    {3}          ,\textcolor{Green}{Yes}
    10,     $id_{11}$,    products,    0.945,    {3}          ,\textcolor{Green}{Yes}
    11,     $id_{12}$,    products,   0.945,    {3}        ,\textcolor{Green}{Yes}
    12,     $id_{13}$,    products,    0.945,    {3}          ,\textcolor{Green}{Yes}
    13,     $id_{14}$,    products,    0.944,    {3}       ,\textcolor{Green}{Yes}
    14,     $id_{15}$,    products,    0.943,    {3}         ,\textcolor{Green}{Yes}
    15,     $id_{16}$,    products,    0.942,     {3}         ,\textcolor{Green}{Yes}
    16,     $id_{17}$,    products,    0.942,   {3}          ,\textcolor{Green}{Yes}
    17,     $id_{18}$,    products,    0.942,    {3}          ,\textcolor{Green}{Yes}
    18,     $id_{19}$,    products,    0.941,   {3}          ,\textcolor{Green}{Yes}
    19,     $id_{20}$,    products,    0.941,   {3}          ,\textcolor{Green}{Yes}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    52,     $id_{53}$,    nutrients,    0.891,                 ,\textcolor{Red}{No}
    $\vdots$,     ,    $\vdots$,    ,              $\vdots$,
    97,     $id_{98}$,    products,    0.881,    {3}          ,\textcolor{Green}{Yes}
    98,     $id_{99}$,    products,    0.881,    {3}          ,\textcolor{Green}{Yes}
    99,     $id_{100}$,    products,    0.880,    {3}          ,\textcolor{Green}{Yes}

}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment3-base-tables:analyst-cv}
                Experiment \ref{advanced-experiment:3} result tuple No.\texttt{2} vs. related \textbf{base tables} with \textbf{Column Vectors} - an analyst's view.
                A subset of the Top-100 tuples from the related base tables, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Column Vectors method.
                }
        }
\end{table}

==> tables/experiment3/base_tables_analyst-tv.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.7,max=0.8, textcolor=white}, format index, format analyst, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     tuple-id, related-table,      {Similarity},      lineage-level,  Lineage 
    0,     $id_1$,    products,    0.969,    {1, 2, 3}          ,\textcolor{Green}{Yes}
    1,     $id_2$,    nutrients,     0.898,    {2}          ,\textcolor{Green}{Yes}
    2,     $id_3$,    nutrients,    0.865,              ,\textcolor{Red}{No}
    3,     $id_4$,    nutrients,    0.848,              ,\textcolor{Red}{No}
    4,     $id_5$,    nutrients,    0.845,             ,\textcolor{Red}{No}
    5,     $id_6$,    nutrients,    0.833,          ,\textcolor{Red}{No}
    6,     $id_7$,    nutrients,    0.831,              ,\textcolor{Red}{No}
    7,     $id_8$,    nutrients,    0.830,              ,\textcolor{Red}{No}
    8,     $id_9$,    nutrients,    0.826,              ,\textcolor{Red}{No}
    9,     $id_{10}$,    nutrients,    0.824,               ,\textcolor{Red}{No}
    10,     $id_{11}$,    nutrients,    0.818,              ,\textcolor{Red}{No}
    11,     $id_{12}$,    nutrients,   0.812,               ,\textcolor{Red}{No}
    12,     $id_{13}$,    nutrients,    0.810,              ,\textcolor{Red}{No}
    13,     $id_{14}$,    serving\_size,    0.810,       {3}       ,\textcolor{Green}{Yes}
    14,     $id_{15}$,    nutrients,    0.801,              ,\textcolor{Red}{No}
    15,     $id_{16}$,    nutrients,    0.791,              ,\textcolor{Red}{No}
    16,     $id_{17}$,    nutrients,    0.760,              ,\textcolor{Red}{No}
    17,     $id_{18}$,    nutrients,    0.751,              ,\textcolor{Red}{No}
    18,     $id_{19}$,    nutrients,    0.750,              ,\textcolor{Red}{No}
    19,     $id_{20}$,    nutrients,    0.742,              ,\textcolor{Red}{No}


}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment3-base-tables:analyst-tv}
                Experiment \ref{advanced-experiment:3} result tuple No.\texttt{2} vs. related \textbf{base tables} with \textbf{Tuple Vectors} - an analyst's view.
                Top-20 tuples from the related base tables, ranked by similarity. Tuple ID contains unique ids of the tuples in question, so that an analyst can quickly retrieve them from the DB. Origin Table is the table name of the tuple's origin. Lineage Level(s) and Lineage show additional meta-data, only known in hindsight (not available to an analyst during lineage querying) to showcase the effectiveness of the Tuple Vectors method.
                }
        }
\end{table}

==> tables/experiment3/base_tables_stats.tex <==
\begin{table*}
\centering
\begin{adjustbox}{width=\textwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.32,max=1.0}, format index, format stats-table1-exp3, format manufacturer, format method,
    col sep=comma,
    /pgfplots/colormap={orange}{
        rgb255(0cm)=(255,245,235);
        rgb255(1cm)=(253,141,60)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    
    index,  Provenance Method,       manufacturer, name, Total, Length-L1, Length-L2, Length-L3,  {1.00$^{Top}$},            {0.75$^{Top}$},        {0.50$^{Top}$},        {0.25$^{Top}$}, Recall-L1, Recall-L2, Recall-L3
    0, Tuple Vectors, conagra brands, healthy choice microwaveable chicken and rice soup, 3571, 1, 2, 3570, 0.172, 0.173, 0.180, 0.199, 1, 1, 0.172
    1, , conagra brands, marie callenders cheesy chicken and rice dinners, 3571, 1, 2, 3570, 0.148, 0.154, 0.162, 0.213, 1, 1, 0.148
    2, , general mills sales inc, annies homegrown organic vegan mac elbow rice pasta sauce, 4000, 1, 2, 3999, 0.183, 0.175, 0.167, 0.162, 1, 1, 0.183
    3, , general mills sales inc, old el paso spanish rice, 4000, 1, 2, 3999, 0.186, 0.191, 0.191, 0.160, 1, 1, 0.186
    0, Column Vectors, conagra brands, healthy choice microwaveable chicken and rice soup, 3571, 1, 2, 3570, 0.678, 0.775, 0.918, 0.981, 1, 0.5, 0.678
    1, , conagra brands, marie callenders cheesy chicken and rice dinners, 3571, 1, 2, 3570, 0.679, 0.751, 0.844, 0.968, 1, 0.5, 0.679
    2, , general mills sales inc, annies homegrown organic vegan mac elbow rice pasta sauce, 4000, 1, 2, 3999, 0.674, 0.75, 0.97, 0.991, 1, 0.5, 0.674
    3, , general mills sales inc, old el paso spanish rice, 4000, 1, 2, 3999, 0.666, 0.719, 0.847, 0.873, 1, 0.5, 0.666
}
\end{adjustbox}
\textbf{\caption{\label{tab:experiment3-base-tables:precision-and-recall}
                Experiment \ref{advanced-experiment:3} query results vs. related base tables (\texttt{products}, \texttt{nutrients} and \texttt{serving\_size}).
                A comparison of different approximate lineage computation methods on the query-result tuples. Total Lineage Size is the size of the exact distant lineage for a result tuple (containing only tuples from the related base tables). Similarly, L[$i$] Lineage Size is the size of the $i^{th}$ lineage level. $p^{Top}$ Precision shows the precision of various methods for the top $p\cdot|Total Distant Lineage|$ tuples in the approximate lineage. For example, 0.50$^{Top}$ is the precision for the top 1785 ($=0.5\cdot3571$) tuples in the approximate lineage of the first result tuple. L[$i$] Recall shows the $i^{th}$ lineage level recall as described in section \ref{sec:recall}.
                }
        }
\end{table*}

==> tables/res1.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.7,max=1.0, textcolor=white}, format index, format table, format userId, format movieId, format tag, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     userId, movieId,               tag,       {Similarity}      ,Lineage              
    0,     282405,    164909 (La La Land),    music ,     0.951796         ,\textcolor{Green}{Yes}
    1,     282405,    152081 (Zootopia),      funny ,      0.941796        ,\textcolor{Green}{Yes}
    2,     282405,    177765 (Coco),          music ,     0.891501 	       ,\textcolor{Red}{No}   


}
\end{adjustbox}

==> tables/res2.tex <==
\begin{adjustbox}{width=\columnwidth,center}
\pgfplotstabletypeset[
    color cells={min=0.7,max=1.0,  textcolor=white}, format index, format table, format userId, format movieId, format tag, format Lineage,
    col sep=comma,
    /pgfplots/colormap={purple}{
        rgb255(0cm)=(239,237,245);
        rgb255(1cm)=(106,81,163)},
    assign column name/.code=\pgfkeyssetvalue{/pgfplots/table/column
        name}{{\textbf{#1}}},
]{
    index,     userId, movieId,               tag,       {Similarity}                    ,Lineage       
    0,     282405,    152081 (Zootopia),    funny ,     0.896420          ,\textcolor{Green}{Yes}
    1,     282405,    164909 (La La Land),      music ,      0.882717          ,\textcolor{Green}{Yes}
    2,     282405,    152081 (Zootopia),          acceptance ,     0.862564           ,\textcolor{Red}{No}   	


}
\end{adjustbox}
